An Introduction to Probabilistic Programming

This book is a graduate-level introduction to probabilistic programming. It not only provides a thorough background for anyone wishing to use a probabilistic programming system, but also introduces the techniques needed to design and build these systems. It is aimed at people who have an undergraduate-level understanding of either or, ideally, both probabilistic machine learning and programming languages. We start with a discussion of model-based reasoning and explain why conditioning is a foundational computation central to the fields of probabilistic machine learning and artificial intelligence. We then introduce a first-order probabilistic programming language (PPL) whose programs correspond to graphical models with a known, finite, set of random variables. In the context of this PPL we introduce fundamental inference algorithms and describe how they can be implemented. We then turn to higher-order probabilistic programming languages. Programs in such languages can define models with dynamic computation graphs, which may not instantiate the same set of random variables in each execution. Inference requires methods that generate samples by repeatedly evaluating the program. Foundational algorithms for this kind of language are discussed in the context of an interface between program executions and an inference controller. Finally we consider the intersection of probabilistic and differentiable programming. We begin with a discussion of automatic differentiation, and how it can be used to implement efficient inference methods based on Hamiltonian Monte Carlo. We then discuss gradient-based maximum likelihood estimation in programs that are parameterized using neural networks, how to amortize inference using by learning neural approximations to the program posterior, and how language features impact the design of deep probabilistic programming systems.

==> sections/advanced-hmc.tex <==
% !TEX root =  ../pp-tutorial-ftml.tex

We introduced Hamiltonian Monte Carlo in Section~\ref{sec:hmc} as a graph-based inference approach,
and variational inference in Section~\ref{sec:eval-bbvi} as evaluation-based inference in the FOPPL;
neither of these we revisited in Chapter~\ref{ch:eval-two} as HOPPL inference algorithms.
This is not because these algorithms are fundamentally difficult to adopt as HOPPL evaluators ---
in fact, it is straightforward to convert the BBVI evaluator in Algorithm~\ref{alg:bbvi-eval} to the HOPPL ---
but rather because it is unclear whether these algorithms yield accurate posterior approximations for programs written in the HOPPL.

The particular challenge is the possibility of HOPPL programs to generate an unbounded number of random variables,
where the number of random variables may differ from execution to execution.
Our BBVI evaluator in Section~\ref{sec:eval-bbvi} produces a variational parameter at each random choice encountered during course of execution; for the FOPPL evaluator in which all random variables can be enumerated, this yields a fixed-size set of variational parameters.
The direct approach to translating this algorithm to the HOPPL is to associate a variational parameter with each address $\alpha$ that corresponds to a \sample statement.
However, this can lead to pathological behaviour where certain addresses may {\em never} be encountered even once
while fitting the approximating distribution, although those addresses may still eventually be produced by the program.
A workaround is to consider a variational approximation which is defined by a finite set of approximating distributions, even if the probabilistic program itself can generate an arbitrary number of random variables during its execution;
this can be done by defining equivalence classes over addresses $\alpha$, such that multiple \sample statements share a posterior approximation.
This is particularly sensible for e.g.\ random choices which occur inside a rejection sampler, where multiple calls to the same distribution in the same function really do have the same posterior, conditioned on the fact that the random variable exists in the execution.
However, in general it is difficult to decide automatically which random choices should share the same approximating distribution.
Such systems can be used in practice so long as these mappings can be annotated manually, as for example in \citet{vandemeent2016blackbox}.

Further difficulties arise if attempting to run Hamiltonian Monte Carlo on HOPPL programs.
A Hamiltonian Monte Carlo transition kernel is not designed to run on spaces of varying dimensionality;
instead, it could be used as a conditional update or proposal for a given fixed set of instantiated random variables.
In a reversible jump MCMC setting, the HMC proposal could update these values while an additional alternative transition kernel could propose changes to the dimensionality of the model.
However, this is also difficult to handle automatically in HOPPL programs;
there is not necessarily any fixed parameter which denotes the dimensionality of the model,
which instead depends on the control flow path of a particular execution.
Changing the value of any continuous latent random variable could push the program onto a different branch (e.g.\ by changing the number of iterations of a stochastic recursion), which would then change the dimensionality of the model.
Implementing HMC in a higher-order programming language safely requires explicitly separating the latent random variables into those which are ``structure preserving'' \citep{yang2014generating}, i.e.\ for which a change in value cannot change the dimensionality of the target, from those which may affect control flow.

\cmt{FW}{Give some lead-in to next section}


==> sections/advanced-nesting.tex <==
%One benefit of using an expressive probabilistic programming language 
%is that it makes it possible to develop and reason about complex models, for instance nested models. 
%In particular, such languages can allow exploration of models defined in terms of inference results on other nested models. In such models, latent random variables or likelihood scores 
%are defined by means of the expectations of some functions over those nested models \citep{rainforth2018nesting,rainforth2016pitfalls}. 

In this tutorial we have not provided a HOPPL construct for nesting probabilistic programs. However, embedded languages like Anglican, WebPPL, and Church inevitably tempt such a facility for many reasons including the existence of a porous boundary between the PPL and its host language.  
Nesting, in our terminology, means treating a HOPPL program like a distribution and using it within another HOPPL program as a distribution-type object, analogous to distributions provided as primitives in the language.
In statistics this can correspond to a double intractable inference problem \citep{murray2012mcmc}.
Nesting would seem a natural and perhaps even straightforward thing to do because a HOPPL program denotes a parameterized conditional distribution (one for each set of observed variable values).  As a consequence one might naturally ask why this HOPPL-denoted distribution ought not be treated just as any other distribution value, in the sense that it can be nested and passed as an argument to \hop{sample} and \hop{observe} in an another or outer HOPPL program.
It turns out that this is very tricky to do correctly and that there remain opportunities to design languages and inference algorithm evaluators that do.  

To even discuss this we need to assume the existence of two additional HOPPL features.  One is a syntactic nesting construct; effectively a boundary around a HOPPL program.
The shared \hop{query} syntax that is used to separate Anglican, Church, and WebPPL programs from their host languages is one such example.  
Second, we need to assume the existence of a construct that reifies a HOPPL program into a distribution type.
In Church and WebPPL this is implicitly tied up in the \hop{query} construct itself, specifically \hop{rejection-query} and \hop{enumerate-query}.  
Other examples of this include the theoretically-grounded but impossible \hop{norm} function of \citet{StatonYWHK16}, and the intentionally hidden \hop{conditional} construct from Anglican, which has flaws uncovered and criticized by \citet{rainforth2018nesting}.

Take for example the following hypothetical nesting-HOPPL program.
\begin{foppl}[mathescape]
(let [inner (query [y D]
              (let [z (sample (gamma y 1))]
                (observe (normal y z) D)
               z))
      outer (query [D]
              (let [y (sample (beta 2 3))
                    z (sample (inner y D))]
              [y z D]))]
  (sample (outer D)))  
\end{foppl}
Even the casual meaning of such a program is open to interpretation.  Should the joint distribution over the return value be 
\begin{align*} 
 \pi _ { 1 } ( y , z , D ) &= p ( y ) p ( z | y ) p ( D | y , z )  \\ 
  &= \operatorname { Beta } ( y ; 2,3 ) \Gamma ( z ; y , 1 ) \mathcal { N } \left( D ; y , z ^ { 2 } \right)  
\end{align*}
or
\[
\left.\begin{aligned} \pi _ { 2 } ( y , z , D ) & = p ( y ) p ( z | y , D ) = \frac { p ( y ) p ( z | y ) p ( D | y , z ) } { \int p ( z | y ) p ( D | y , z ) \mathrm dz} \\ & = \frac { p ( y ) p ( z | y ) p ( D | y , z ) } { p ( D | y ) } \neq \pi _ { 1 } ( z , y , D ) \end{aligned}\ ?\right.
\]
The first interpretation is what you would expect if you were to inline the inner query as one can do for a function body in a pure functional language.  While doing such a thing introduces no mathematical complications, it is incompatible with the  conditional distribution semantics we have established for HOPPL programs.  The second interpretation is correct in that it is in keeping with such semantics but introduces the extra marginal probability term $p(D|y)$ which is impossible to compute in the general case, complicating matters rather a lot.  

\citet{rainforth2018nesting} categorizes nesting into three types: ``sampling from the conditional
distribution of another query'' (which we refer to as nested
inference), ``factoring the trace probability of one query
with the partition function estimate of another'' (which we
refer to as nested conditioning), and ``using expectation estimates
calculated using one query as first class variables
in another.''  
While this terminology is rather inelegant (and potentially confusing because it conflates problem and solution differences in the same categorization), the point remains. 
To even do ``nested inference'' one both must pay close attention to \citet{rainforth2017nested} warnings about 
convergence rates for nested sampling  and also utilize sampling methodologies 
that are specifically tailored to this situation \citep{rainforth2018nesting,naesseth2015nested}.


%The model for the agent B in this case includes her knowledge about the agent C,
%but this knowledge is represented by means of an expectation over the model for C. 

%Operationally, such models including other nested models can be understood 
%as samplers that invoke inference algorithms over those nested models while producing a single 
%sample. Invoking an inference algorithm this way is allowed in
%probabilistic programming languages like Anglican, WebPPL and Venture, so that these
%models can be easily expressed in those languages.

Beyond these concerns \citet{StatonYWHK16} also noticed that the posterior distribution fails to be defined in
some models with certain observation distributions because the marginal likelihood of the observation can become infinite \citep{StatonYWHK16,StatonESOP17}. 
Here is a variant of their example.
\begin{foppl}[mathescape, label={pr:bad-nesting}, caption={HOPPL program with undefined posterior}]
(let [x (sample (normal 0 1))
      px (* (/ 1 (sqrt (* 2 pi))) 
            (exp (- (/ (* x x) 2))))]
  (observe (exponential (/ 1 px)) 0)
  x)
\end{foppl}
This program defines a model with prior $p(x) = \mathrm{Normal}(x;0,1)$
and likelihood $p(y|x) = \mathrm{Exponential}(y;1/p(x))$,
and expresses that $y=0$ is observed. The model fails to have a posterior 
because its marginal likelihood at $y=0$ is infinite
\begin{align*}
p(y=0) 
= \int p(x,y=0) \mathrm{d}x 
& = \int p(x)p(y=0|x) \mathrm{d}x 
\\
& = \int p(x) \frac{1}{p(x)} \mathrm{d}x = \infty.
\end{align*}
\citet{StatonYWHK16} argued that the formal
semantics of a language construct for performing inference, such as $\mang{doquery}$ in Anglican, should account for this failure case.  A message of this research to us is that 
when we define a model using the outcome of posterior inference of another nested model,
we should make sure that this outcome is well-defined, because otherwise even a prior
used within an outer model may become undefined. 

%This is on top of the already mentioned concerns raised by \citet{rainforth2017nested} about
%the convergence properties of algorithms that perform multiple inference tasks in a nested
%fashion \citep{rainforth2017nested}. In particular, they studied a naive nested Monte-Carlo algorithm
%that generates a single sample from a model
%after drawing multiple samples from another nested model
%and computes an estimate based on these samples. \citet{rainforth2017nested} point out that 
%the mean square error of this na\"ive nested Monte-Carlo has a very bad convergence rate,
%and demonstrated opportunities for improving it by identifying and exploiting additional properties of the target model.
%, such as linearity
%or Taylor expansion, and to convert the estimation problem over the model into an equivalent one 
%that does not involve a nested use of Monte-Carlo algorithms. 

Currently probabilistic
programming languages perform inference on nested models in a way that is similar to 
the bad na\"ive nested Monte-Carlo identified by \citet{rainforth2017nested} and in a way that is not immune to the problem identified by \citet{StatonYWHK16}, and so they suffer from inefficiencies and, worse, inaccuracies. This suggests a potentially fruitful avenue for future research.

What should be noted is that nested query language constructs, were they to be operationalized efficiently and correctly, allow one to express extremely interesting and complex generative models that can involve mutually recursive theory-of-mind type reasoning, and so on.
Goodman and his colleagues highlight many such 
models for agent interactions that capture agents' knowledge about other agents \citep{stuhlmuller2014reasoning} and many source code examples are available online \citep{forestdb}.

%
%What does it mean to have defquery in the language?  There are applications in which one might wish to compute or estimate, given a fixed budget, the expectation or variance of some latent quantity.  
%\fw{include a sample example}
%Without the ability to perform inference in the language itself these quantities are forever outside scope.  Languages like Anglican, WebPPL, and Venture allow arbitrary nesting of queries despite the fact that there are some problems with the mathematical abstractions represented by such constructs \citep{rainforth2016pitfalls}.
%\fw{here here please!}
%
%Plan:
%\begin{itemize}
%\item Nested inference. Applications. Rainforth's Bayesian experimental design. Goodman's recursive reasoning examples.
%\item Computational challenge. Naive Monte-Carlo approach. Slow convergence. Need to exploit structure of enclosing queries as much as possible. Taylor expansion and Russian roullet estimator.
%\item Semantic challenge. The outcome of inference sometimes undefined. Fully informative interface, i.e., type.  
%\end{itemize}


==> sections/advanced-semantics.tex <==
Programs in probabilistic programming languages correspond to probabilistic models, and characterizing aspects of these models is the goal of inference algorithms. In most cases, the characterization is approximate, and describes the target model only partially. Although such partial description is good enough for many applications, it is not so for the developers of these languages, who have to implement compilers, optimizers, and inference algorithms and need to ensure that these implementations do not have bugs.  For instance an optimizer within a PPL compiler should not change the probabilistic models denoted by programs, and an inference algorithm should be able to handle corner cases correctly, such as Program~\ref{pr:bad-nesting} in Section~\ref{sec:nesting} that does not have a posterior distribution. To meet this obligation, developers need a method for mapping probabilistic programs to their precise meanings, i.e., a strict mathematical description of the denoted probabilistic models. The method does not have to be computable, but it should be formal and unambiguous, so that it can serve as ruler for judging correctness of transformations and implementations.

A formal semantics is such a method. It defines the mathematical meaning of every program in a probabilistic programming language. For instance, the semantics may map
\begin{foppl}[mathescape]
(let [x (sample (normal 0 1))]
  (observe (normal x 1) 2)
  x)
\end{foppl}
to the normalized posterior distribution of the returned latent variable $x$ (namely, $\mathrm{Normal}(x;1,\sqrt{2})$), or to its unnormalized counterpart $\mathrm{Normal}(x;0,1) \times \mathrm{Normal}(2;x,1)$, which comes directly from the joint distribution of the latent $x$ and the observed $y$ that has the value $2$.

A formal semantics is like integration. The integral of a complicated function may be impossible to compute, but its mathematical meaning is clearly defined. Similarly, the semantics might not tell us how to compute a probabilistic model from a given complicated program, but it tells us precisely what the model is.

Giving a good formal semantics to probabilistic programming languages turns out to be very challenging, and even requires revising the measure-theoretic foundation of modern probability theory in some cases. 
These issues can be seen in articles by \citet{BorgstromGGMG13}, \citet{StatonYWHK16}, and \citet{StatonESOP17}.
In the rest of this section, we focus on {\em one} issue caused by so-called higher-order functions, which are functions that take other functions as arguments or return functions as results; 
higher-order function are fully or partially supported by many probabilistic programming languages such as Church, Venture, Anglican, WebPPL and Pyro. 

A good way to understand the issue with higher-order functions is to attempt to build a formal semantics for a language with higher-order functions and
to observe how a natural decision in this endeavor ultimately leads to a dead end. The first step of 
this attempt is to notice that a large class of probability distributions
can be expressed in the HOPPL and most other probabilistic programming languages. In particular,
using these languages, we can express distributions on real numbers that do not have density
functions with respect to the Lebesgue measure, and go easily outside of the popular comfort zone of using
density functions to express and reason about probabilistic models.  
For instance, the HOPPL program
\begin{foppl}[mathescape]
(if (sample (flip 0.5)) 1 (sample (normal 0 1)))
\end{foppl}
expresses a mixture of the Dirac distribution at $1$ and the standard normal distribution,
but because of the Dirac part, this mixture does not have a density function with 
respect to Lebesgue measure. 

A standard approach of formally dealing with such distributions is to use measure theory.
In this theory, we use 
a so called \emph{measurable space}, which is just a set $X$ equipped with a family $\Sigma$ of 
subsets of $X$ that satisfies certain conditions. Elements in $\Sigma$ are called \emph{measurable},
and they denote events that can be assigned probabilities. A representative example of measurable 
space is the set of reals $\mathbb{R}$ together with the family $\mathcal{B}$ of so called Borel sets. 
A probability distribution on $X$ is then defined to be a function from $\Sigma$ to $[0,1]$ satisfying 
certain properties. For instance, the above HOPPL program denotes a distribution that assigns 
\[
        0.5 \times \mathbb{I}(a < 1 < b) + 
        0.5 \times \int_a^b \frac{1}{\sqrt{2 \pi}} \exp\left(\frac{-x^2}{2}\right)\mathrm{d}x
\]
to every interval $(a,b)$. Another important piece of measure theory is that 
we consider only \emph{good} functions $f$ between two measurable spaces $(X,\Sigma)$ and $(X',\Sigma')$
in the sense that the inverse image of a measurable $B \in \Sigma'$ according to $f$
is always measurable (i.e. $f^{-1}(B) \in \Sigma$). These functions are called \emph{measurable functions}.
When the domain $(X,\Sigma)$ of such a measurable function is given a probability distribution, we
often say that the function is a random variable. Using measure theory amounts to formalizing objects 
of interest in terms of measurable spaces, measurable sets, measurable functions 
and random variables (instead of usual sets and functions).

The second step of giving a semantics to the HOPPL is to interpret
HOPPL programs using measure theory. It means to map HOPPL programs to measurable functions,
constants in measurable spaces, or probability distributions. Unfortunately, this
second step cannot be completed because of the following impossibility result 
by \cite{aumann:functionspaces}:
\begin{theorem}[Aumann]
        Let $F$ be the set of measurable functions on $(\mathbb{R},\mathcal{B})$. Then,
        no matter which family $\Sigma$ of measurable sets we use for $F$, we cannot make
        the following evaluation function measurable:
        \begin{align*}
                \mathit{app} & : F \times \mathbb{R} \to \mathbb{R}
                \\
                \mathit{app}(f,r) & = f(r).
        \end{align*}
        Here we assume that $\mathcal{B}$ is used as a family of measurable sets for $\mathbb{R}$
        and that $F \times \mathbb{R}$ means the standard cartesian product of
        measurable spaces $(F,\Sigma)$ and $(\mathbb{R},\mathcal{B})$.
\end{theorem}
The result implies that the HOPPL function 
\begin{hoppl}[mathescape]
        (fn [f x] (f x))
\end{hoppl}
cannot be interpreted as a measurable function, and so it lives outside
of the realm of measure theory, regardless of what measurable
space we use for the set of measurable functions on $(\mathbb{R},\mathcal{B})$. We thus have to look for 
a more flexible alternative than measure theory.

Finding such an alternative has been a topic of active research. Here we
briefly review a proposal by Heunen, Kammar, Staton and Yang~\cite[]{HeunenKSY17}.
The key of the proposal lies in their new formalization of probability theory
that treats the random variable as a primary concept and axiomatizes it directly.
Contrast this with the situation in measure theory where measurable sets
are axiomatized first and then the notion of random variable is derived from this
axiomatization (as measurable function from a measurable space with a probability
distribution). It turns out that this shift of focus 
leads to a new notion of good functions, which
is more flexible than measurability and lets one 
interpret HOPPL programs, such as the 
application function from above, as good functions.

More concretely, \citet{HeunenKSY17} axiomatized a set $X$ equipped with a collection of
$X$-valued random variables in terms of what they call \emph{quasi-Borel space}. 
A quasi-Borel space is a pair of a set $X$ and a collection $M$ of functions 
from $\mathbb{R}$ to $X$ that satisfies certain conditions, such as
all constant functions being included in $M$. Intuitively, the functions in $M$ 
represent $X$-valued random variables, and they use real numbers as
random seeds and are capable of converting such random seeds
to values in $X$. The measurable space $(\mathbb{R},\mathcal{B})$ is one of the 
best-behaving measurable spaces, and using real numbers in this space as 
random seeds ensures that quasi-Borel spaces avoid pathological cases in measure theory.
A less exciting but useful quasi-Borel space is $\mathbb{R}$ with 
the set $M_{\mathbb{R}}$ of measurable functions from $\mathbb{R}$ to itself,
which is an example of quasi-Borel space generated from a measurable space.
But there are more exotic, interesting quasi-Borel spaces that do not arise from 
this recipe. 

Heunen et al.'s axiomatization regards a function $f$ from 
a quasi-Borel space $(X,M)$ to $(Y,N)$ as good if $f \circ r \in N$ for all $r \in M$; 
in words, $f$ maps a random variable in $M$ to a random variable in $N$. They have shown
that such good functions on $(R,M_{\mathbb{R}})$ themselves form a quasi-Borel space when
equipped with a particular set of function-valued random variables. Furthermore,
they have proved that the application function \mang{(fn\ [f\ x]\ (f\ x))} from above
is a good function in their sense because it
 maps a pair of such function-valued random variable and $\mathbb{R}$-valued random variable
to a random variable in $M_{\mathbb{R}}$.  

Heunen et al.'s axiomatization has been used to define the semantics of probabilistic programming
languages with higher-order functions and also to validate inference algorithms for such languages.
For interested readers, we suggest \citet{HeunenKSY17} as well as \citet{ScibiorKVSYCOMH18}.


==> sections/advanced-symbolic.tex <==
Throughout the tutorial, we focused on inference algorithms that are designed to analyze nearly all programs in a target probabilistic programming language. Opportunistic techniques that work only for particular programs also exist, and symbolic methods~\cite{NoriHRS14,narayanan2016probabilistic,gehr2016psi,MurrayLKBS18} are good examples. These methods use mathematical properties of probability distributions and program semantics, and transform parts of a given program to those that are friendlier to a subsequent inference algorithm than the original. They are usually implemented inside a compiler for the probabilistic programming language, and applied to all the programs in the language automically during compilation time.

One general theme behind multiple symbolic methods is to propagate information about observed random variables backward through a program, so that the information becomes available when latent variables get sampled in the program. The propagated information then helps an inference algorithm to pick effective proposal distributions for latent variables. Sometimes it even enables the compiler to replace the prior distribution of a latent variable by the posterior with respect to some observation. 

For instance, consider the following FOPPL program:
\begin{foppl}[mathescape]
(let [x1 (sample (gamma a b))]
  (let [x2 (sample (normal x1 1))]
    (observe (poisson x1) y)
    (list x1 x2)))
\end{foppl}
The observe statement provides information about the latent variable \fop{x1}. A symbolic method can may propagate this information to the sample statement of \fop{x1}. First, it swaps the observe statement and the sampling of \fop{x2}:
\begin{foppl}[mathescape]
(let [x1 (sample (gamma a b))]
  (observe (poisson x1) y)
  (let [x2 (sample (normal x1 1))]
    (list x1 x2)))
\end{foppl}
This transformation preserves the semantics of the program (i.e., the joint distribution of the latent and observed variables). In fact, commuting two commands in a FOPPL program without any data dependency preserves the semenatics. Next, the method interchanges the sampling of \fop{x1} with the observe statement using a well-known equation about the conjugacy between gamma prior and poisson likelihood:
\begin{foppl}[mathescape]
(let [p (/ 1 (+ b 1))]
  (observe (negative-binomial a p) y)
  (let [x1 (sample (gamma (+ a y) (+ b 1)))]
    (let [x2 (sample (normal x1 1))]
      (list x1 x2))))
\end{foppl}
The used equation is:
\begin{multline*}
\mathrm{Gamma}(x_1;a,b) \cdot \mathrm{Poisson}(y; x_1)
= {}
\\
\mathrm{Gamma}(x_1;a+y,b+1) \cdot \mathrm{NegativeBinomial}\Big(y; a, \frac{1}{b+1}\Big).
\end{multline*}

Note that the symbolic method completes posterior inference in this case. The program after the two-step tranformation implements a sampler for the posterior $p(x_1,x_2|y)$ of the original program, and its observe statement specifies the marginal likelihood $p(y)$ directly:
\[
        p(y) = \mathrm{NegativeBinomial}(y; a, \frac{1}{b+1}).
\]
This is not a norm, though. Typically, a symbolic method is not powerful enough to complete posterior inference for itself, or the posterior of a given probabilistic program is simply too complicated to be inferred completely by a symbolic approach. As a result, most symbolic methods are used as preprocessors of generic inference algorithms.

There are two notable exceptions to the use of a symbolic method as a preprocessor. The first is probabilistic programming systems that aim at computing posterior distributions exactly. These systems employ sophisticated symbolic techniques, often involving powerful computer algebra systems, such as Maple. Hakaru~\citep{narayanan2016probabilistic} and PSI Solver~\citep{gehr2016psi} are representative examples. The second is probabilistic programming systems that implement so called delayed sampling~\citep{MurrayLKBS18,MurrayS18,KudlickaMRS19}. Such a system uses a symbolic method not before but during the execution of a sampling-based inference algorithm. The system monitors the values sampled by the algorithm, looks for an opportunity for symbolic simplification, such as integration of a latent variable, and carries out such simplification upon the detection of the opportunity. Birch~\citep{MurrayS18} is a good example that implements delayed sampling and this on-the-fly symbolic simplification.


==> sections/advanced.tex <==
% !TEX root =  ../pp-tutorial-ftml.tex
% !TEX spellcheck = en_US

So far in this tutorial we have looked at how to design first-order and higher-order probabilistic programming languages,
and provided a blueprint for implementation of automatic inference in each.
In this chapter, we change direction, and describe some recent advances around current questions of research interest in the field at the time of writing.

We look in a few different directions, 
for instance
% considering the challenges in implementing Hamiltonian Monte Carlo and variational inference within the HOPPL, 
using symbolic techniques for better inference, and
implementing expressive models by recursively nesting probabilistic programs. We conclude with an introduction to formal semantics for probabilistic programming languages.

%	
%\section{Hamiltonian Monte Carlo and Variational Inference}
%\input{sections/advanced-hmc}

\section{Symbolic Methods}
\label{sec:symbolic}
\input{sections/advanced-symbolic}

\section{Nesting}
\label{sec:nesting}
\input{sections/advanced-nesting}

\section{Formal Semantics}
\label{sec:semantics}
\input{sections/advanced-semantics}


	



==> sections/deep-faithful-inverses.tex <==
% !TEX root =  ../pp-tutorial-ftml-wip.tex

%\subsection{Reasoning About Faithful Inverses}

The two strategies for amortization that we have discussed so far have defined proposals that generate samples in the same order as in the generative model. This was true for WebPPL-style proposals, which employ a \hop{(propose $d_p$ $d_q$)} form that requires both a prior $d_p$ and a proposal $d_q$ as its arguments. It was also true for PyProb-style proposals, in which a recurrent network constructs a proposal $d_q$ each time an expression \hop{(sample $\alpha_0$ $d_p$)} is evaluated in the model. In both cases, the proposal $q(x \mid Y, \pa_p(x), \phi)$ for a particular variable $x$ can depend on the data $Y$, as well as on upstream variables in the generative model $\pa_p(x)$, but not on any  downstream variables. %However, this dependency structure is often not optimal. 

A limitation of conditioning on preceding samples is that not all preceding preceding variables may in fact be relevant to the current proposal. This means that we are imposing a greater burden on the neural network, which must now learn which preceding variables are informative in the context of the current proposal. Moreover, in this design it is not possible to make use of correlations between the current variable and variables that are instantiated later in the execution.

In the context of languages like the FOPPL, where programs can be compiled to a graphical model, the proposal need not have the same dependency structure as the program prior. In this setting, the proposal can be any graphical model, as long as this model has the same unobserved random variable nodes as the prior. The question that then arises is how we can choose an inverse model that appropriate makes use of and conditional dependence and independence in the the original model.

This question has given rise to a line of work on constructing inverses of graphical models. A simple approach is to invert the direction of each edge in the generative model. Since parents in a graphical model are correlated when conditioned on their children, we can introduce edges in the inverse model between parents in the generative model that allow us to capture such correlations. This approach was originally proposed by \citet{stuhlmueller2013learning}, and later applied to learn proposals using sleep-phase updates by \citet{paige2016inference}. 

\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.7\linewidth]{figs/webb-neurips-2018-fig1-crop.pdf}
\end{center}
\caption{Example of model inverses (from \citet{webb2017faithful}). \emph{(Left)} A generative model in which two branches are independent under the prior, but correlated under the posterior. \emph{(Middle)} Inversion proposed by \citet{stuhlmueller2013learning}, in which branche are uncorrelated in the inference model. \emph{(Right)} Faithful inversion, which mirrors the correlation structure in the posterior. 
[BROOKS: I think we could use a better figure here!]}
\end{figure}

This simple strategy for inversion can however give rise to conditional independencies in the inference model that are not present in the posterior of the generative model. This means that the learned proposal will never be able to faithfully capture correlations in the posterior, even when edges are parameterized using neural networks.

[TODO FINISH DISCUSSION OF FAITHFUL INVERSES]


==> sections/deep-prob-prog-intro.tex <==
% !TEX root =  ../pp-tutorial-ftml-wip.tex

Up to this point in this book we have focused mainly on two things: 1) the probabilistic programming language design space and 2) inference algorithms.  %This chapter shifts focus rather a lot.  
We have more-or-less assumed that there is a fully specified program in which we wish to perform inference and that we will be doing inference once, since we only have one set of observed data.
This is, in fact, true in a variety of circumstances; notably when doing traditional Bayesian statistical analyses of small data or when doing high fidelity simulation-based studies of particular phenomena. We have also assumed that it does not particularly matter how long inference will take, as long as we can produce high-quality inference results given our computational budget. This chapter pushes past these assumptions.


%We have also assumed that it does not really matter how long inference will take.  In particular, we have assumed that we will be doing inference once per program, and that we would like to have algorithms that produce the highest quality inference results possible in such one-time-only inference scenarios.  

In Chapter~\ref{ch:introduction} we motivated the whole of probabilistic programming by suggesting the utility of probabilistic programming languages and techniques for solving modern artificial intelligence (AI) and machine learning (ML) problems.  This chapter builds on what we have developed so far in this book, addressing issues that commonly arise in ML and AI applications.  

In particular, ML and AI applications are typified by several characteristics that are different to those that we have considered so far in our pedagogical examples.  One, ``big data'':  the existence of huge amounts of data; sometimes labeled, sometimes unlabelled, and sometimes partially labeled.  Two, what we will describe as ``non-programmability'':  the idea that, for instance, in many AI and ML applications it is  inconceivable how to write down a fully specified generative program that describes the entire data generation process.   And three, a ``rapid inference'' requirement:  in many if not all interesting AI and ML applications inference will be repeated and must be fast if it is to be valuable at all.  The techniques covered in this chapter address all of these points.

\section{Examples}
\subsection*{Bayesian Neural Networks}
To build some intuition about such ML/AI application characteristics, first refer back to the very simple Bayesian neural network example program in Chapter~\ref{ch:foppl}, Program~\ref{foppl:bnn_edward}, which framed parameter ``learning'' in a neural network as inference in, effectively, a generative model of neural network parameters.  This program generated the weights of a neural network from a standard prior (corresponding to ``weight decay'' or L2 regularization) and observed the output value of a number of input/output observation pairs (corresponding to an L2 regression loss) given the input passed through the neural network.   The input/output relationship of the data inlined in Program~\ref{foppl:bnn_edward} is so simple that it can be deduced directly by simply looking at the data: output equals input squared.  The triviality of this example made writing the program compact and illuminating with respect to the design of the FOPPL but  may have obfuscated the important points that we address in this chapter.  Simply considering a larger scale, generic version of this program/problem will help characterize two of these points.  Consider the pseudo-code in Program~\ref{foppl:generic_bnn}.  This is a generic program that takes a large amount, \mang{N}, of data $Y_1, \ldots, Y_N$ consisting of input/label pairs and generates a posterior distribution over the weights $\theta$ of a neural network. 

\begin{foppl}[mathescape,caption={A Generic Bayesian Neural Network for Classification},label=foppl:generic_bnn,float=tbp,floatplacement=thbp]

(defn sample-weights [] $\ldots$)

(defn neural-network [weights input] $\ldots$)

(let [Y [$\ldots$] ;; [[input1 label1] [input2 label2] $\ldots$] 
      N $\ldots$     ;; number of training pairs
      $\theta$ (sample-weights)]
  (foreach N 
    [$Y_i$ Y]
    (let [input (get $Y_i$ 0)
          label (get $Y_i$ 1)] 
      (observe 
        (discrete (neural-network $\theta$ input)) 
        label)))
  X)  
\end{foppl}

%\begin{foppl}[mathescape,caption={A Generic Bayesian Neural Network for Classification},label=foppl:generic_bnn,float=tbp,floatplacement=thbp]
%
%(defn sample-weights [] $\ldots$)
%
%(defn neural-network [weights input] $\ldots$)
%
%(let [input [$\ldots$]
%      label [$\ldots$]
%      N $\ldots$
%      weights (sample-weights)]
%  (foreach N 
%    [x input 
%     y label] 
%    (observe (discrete (neural-network weights x)) y))
%  weights)  
%\end{foppl}

Program~\ref{foppl:generic_bnn} illustrates two of the characteristics of ML/AI applications.  First, it illustrates conditioning on a large amount of data.  This has ramifications we will consider with respect to whether or not we should treat $\theta$ as a parameter for which we should compute a point estimate or whether we should continue, as we have throughout the entire book until now, to treat it as a latent variable for which we should compute an approximate posterior. And second, the relationship from input to label, particularly if the inputs live in, for instance, the space of images, and the labels live in, for instance, the space of object class identities, is impossible to program manually (whereas it was not just conceivable but even trivial in Program~\ref{foppl:bnn_edward}).   In other words the \mang{neural-network} function which takes  \mang{weights} and \mang{input} and produces, here, softmax weights for the parameters of categorial (or cross-entropy) loss can be thought of as an otherwise impossible to code program fragment; a part of the model which we would like to learn.  %Assume that some architecture of the neural network is given (e.g.~convolutional with three layers, some number of filters, some kind of pooling, etc.), but the parameters of this neural network are not, and what we want/aim to do is to learn the parameters of this program fragment (or distribution over them as is the case thusfar) so that the rest the whole program ``makes sense.''  
This is, in a sense, what model learning is about. 

\subsection*{Model Predictive Control}
%
\begin{foppl}[mathescape,caption={Model-Predictive Control via Inference},label=foppl:generic_rl_state_transition_model,float=tbp,floatplacement=thbp]
;; Markov decision process (MDP)
(defn next-state-dist [$s_t$ $a_t$] $\ldots$ $p(s_{t+1}|s_{t},a_t)$)
(defn reward [$s_t$ $a_t$] $\ldots$)
(defn allowed-action-dist [$s_t$] $\ldots$ $p(a_t|s_{t})$)

(defn step [t s_and_a]
  (let [s (get s_and_a 0)
        a (get s_and_a 1)
        next_s (sample (next-state-dist s a))
        next_a (sample (allowed-action-dist next_s))]
     (observe 
        (bernoulli (exp (- (reward next_s next_a)))) 
        true) ;; $y_t$ =  true
     [next_s next_a]))

(let [$T$ 10 ;; planning horizon
      $a_t$ (sample (allowed-action-dist $s_t$))]
   (observe 
     (bernoulli (exp (- (reward $s_t$ $a_t$))))
     true)
   (loop $T$ [$s_t$ $a_t$] step)
   $a_t$)
\end{foppl}
% ;; assume current state $s_t$ already bound 
% (defn equilibrium-state-dist [$s$] $p(s)$)
%      _ (observe (equilibrium-state-dist) $s_t$)
While Program~\ref{foppl:generic_bnn} highlights the first two AI/ML problem characteristics we address in this chapter, it does not require rapid, repeated inference. Program~\ref{foppl:generic_rl_state_transition_model} does.  This program frames action selection in model predictive control setting as an inference problem.  This program frames the Markov decision process control problem of selecting action $a_t$ when in state $s_t$ via inference in the joint distribution
%
\begin{align}
p(a_t,s_t,&\tau,y_{t:t+T}) = p(s_t)p(a_t|s_t) p(y_t|s_t,a_t) 
\\
& {} \times 
        \prod_{i=1}^{T} 
        p(s_{t+i}|s_{t+i-1},a_{t+i-1})
        p(a_{t+i}|s_{t+i}) 
        p(y_{t+i}|s_{t+i}, a_{t+1}) 
        \nonumber
\end{align} 
%
where $\tau = \{s_{t+1}, a_{t+1}, \ldots, s_{t+T}, a_{t+T}\}$.  Here $Y = \{s_t,y_{t:t+T}\}$ are the observations on which we will condition and $X = \{s_{t+1:t+T},a_{t:t+T}\}$ are the latent variables, the marginal conditional distribution of $a_t$ being of particular interest.  The $y_{t:t+T}$'s are auxiliary Boolean variables that always take the value \mang{true}, and the variables are given distributions with parameters that put the reward in the ``right places'' mathematically speaking in following expressions. The conditional distribution of 
%
\begin{align}
p(&a_t,\tau|s_t, y_{t:t+T} = \vec{\mang{true}}) \\
        &\propto  p(a_t|s_t)e^{r(s_t, a_t)} \prod_{i=1}^{T} 
        p(s_{t+i}|s_{t+i-1},a_{t+i-1})p(a_{t+i}|s_{t+i}) 
        e^{r(s_{t+i}, a_{t+i})} 
        \nonumber
\end{align} 
%
contains the marginal $p(a_t|s_t, y_{t:t+T} = \vec{\mang{true}})$ which is the ``optimal'' distribution over the action to take at time $t$ given an undiscounted ``planning'' horizon of time $T$.  This choice is optimal in the sense that 
\begin{align}
\log p(&a_t|s_t, y_{t:t+T} = \mang{true}) \\
%%&=  {r(s_t, a_t)} + \log \left( \int e^{r(s_{t+i}, a_{t+1})} p(s_{t+i}|s_{t+i-1},a_{t+i-1}) p(a_{t+i}|s_{t+i}) d\tau \right) \\
        &=  \log p(a_t|s_t) + {r(s_t, a_t)}  + \log\left( \mathbb{E}_{p(\tau|a_t,s_t)}\left[\prod_{i=1}^T e^{r(s_{t+i}, a_{t+i})}\right]\right) \label{eq:1bf}\\
        &\geq \log p(a_t|s_t) + {r(s_t, a_t)} + \mathbb{E}_{p(\tau|a_t,s_t)}\left[\sum_{i=1}^T r(s_{t+i}, a_{t+i})\right] \label{eq:1af} \\
        &\approx  \log p(a_t|s_t) + r(s_t, a_t) + Q(s_t,a_t)
\end{align} 
where $p(a_t|s_t)$ is usually the uniform over all choices of $a_t$ and does not affect the optimality, $r(s_t, a_t)$ is the instantaneous reward for taking action $a_t$, and $Q(s_t,a_t)$ is the expected reward ahead, integrating over future states of the world
assuming that you have no a priori preference over subsequent actions and the world transitions according to your model $p(s_{t+1}|s_{t},a_t)$ of it.  We assume positive rewards and use Jensen's inequality to go from \eqref{eq:1bf} to \eqref{eq:1af}.

This application, while a bit involved as an example, directly highlights the most genuine kind of ML/AI application inference runtime requirement.  Of course there are other ways to learn and choose how act in the world besides model-predictive control.   However, any agent that does use inference for model-predictive control for action selection cannot wait around for a long time while an estimate of $p(a_t|s_t,y_{t:t+T})$ is approximated before acting.   And such an agent would need to repeatedly, not just one-time, solve this inference problem.

Careful readers will note that $s_t$ is not bound in Program~\ref{foppl:generic_rl_state_transition_model}.  This is because this is a conditional generative model and it can safely be assumed that this probabilistic program would be executed in a context in which $s_t$ is known and would be provided to the model at inference time.
\subsection*{Variational Autoencoder}

%(defn softplus [x] (log (+ 1 (exp x))))
\begin{foppl}[escapeinside={/*!}{!*/},mathescape,caption={Variational Auto-Encoder},label=foppl:vae,float=tbp,floatplacement=thbp]
;; q, the "encoder"
(defn q-x [$\phi$ $Y_n$] 
  (let [h (nn_q_1 $Y_n$ $\phi$)
        mu (nn_q_2 h $\phi$)
        sigma-sq (vsoftplus (nn_q_3 h $\phi$))]
     (diag-mvn mu sigma-sq)))
     
(defn inference-network [$\phi$ $Y_n$]
  (sample (q-x $\phi$ $Y_n$)))
  
;; p, the "decoder"
(defn generative-model [$\theta$ $Y_n$]
  (let [$X_n$ (sample (diag-mvn $\theta$))
        h (nn_p_1 $X_n$ $\theta$)
        mu (nn_p_2 h $\theta$)
        sigma-sq (softplus (nn_p_3 h $\theta$))]
     (observe (diag-mvn mu sigma-sq) $Y_n$)))          
\end{foppl}

While not an application per se, the variational autoencoder (VAE) model family \citep{rezende2014stochastic,kingma2014auto} arguably is what led to the confluence of probabilistic programming and deep learning which we cover in this chapter.  Variational autoencoders consist of both a generative model which transforms a random vector into a likelihood over some observation space and an amortized inference artifact that performs approximate inference in constant time.  While exactly what this inference network is will not be clear until later in the chapter, you can think of it as replacing the asymptotically convergent inference {\em algorithms} that we have thusfar discussed throughout this book with a constant-time approximate algorithm.  

Program~\ref{foppl:vae} shows program fragments corresponding to both parts of a generic VAE, a generative model or ``decoder'' \mang{p} and an inference network or ``encoder'' \mang{q}.  All variables in Program~\ref{foppl:vae} should be read as being vector valued, \mang{vsoftplus} should be read as the broadcasting of the softplus function $f(x) = \log(1+\exp(x))$ across the dimensions of the argument (i.e., the pointwise application of the softplus to the input vector), all of the \mang{nn_q}'s and \mang{nn_p}'s should be read as neural networks of some structure whose weights are subsets of $\phi$ and $\theta$ respectively, and \mang{diag-mvn} is a multivariate normal distribution with a diagonal covariance matrix whose diagonal elements are given by the vector \mang{sigma-sq}.  For concreteness you could imagine that $Y_n$ is a vectorized, transformed grayscale image and $X_n$ is a, say, 64 dimensional vector.

VAEs bring together all of the characteristics of AI/ML problems in the probabilistic programming context.  The role of the encoder is explicitly to perform rapid amortized inference.  The decoder is a partially specified generative model.  Only the structure of the generative model is provided; the neural network architecture and the choice of prior and likelihood distribution types.  The rest must be learned from data.  And more clearly than any of the previous examples, the very idea of learning generative model parameters from the data requires multiple observations, in many cases ``big data.''  In Program~\ref{foppl:vae} the decoder is in the form of the programs we have seen throughout this text.  Inference in this program would return the posterior distribution over \mang{x} given \mang{y} for each value of $\theta$.  But without some way to do model parameter learning, inference in such a generative model is non-sensical.

Deep probabilistic programming systems can largely accurately be thought of as languages for specifying richly structured variational auto-encoders where both the encoder (also sometimes called a ``guide'') and the generative model are {\em both} considered part of a probabilistic program.

\subsection*{Structured VAE - A Running Pedagogical Example}
\begin{foppl}[mathescape,caption={Non-Interleaved Inference Network and Generative Model},label=foppl:pyro-like-model,float=tbp,floatplacement=thbp]
;; inference network, q, params
;; i.e. (def $\phi$ [$\ldots$, $\ldots$]) 
(defn get-$\phi_z$ [$\phi$] (get $\phi$ 0))
(defn get-$\phi_\mu$ [$\phi$] (get $\phi$ 1))

;; inference network q
(defn q-z [$\phi$ $Y_n$ $X_n$ $S$] $\ldots$)
(defn q-mu [$\phi$ $Y_n$ $X_n$ $S$] $\ldots$)

(defn inference-network [$\phi$ $Y_n$]
  (let 
     [[q_z1 q_s1] (q-z (get-$\phi_z$ $\phi$) $Y_n$ [] nil) 
      $z_1$ (sample (q_z1)) 
      [q_z2 q_s2] (q-z (get-$\phi_z$ $\phi$) $Y_n$ [$z_1$] q_s1)
      $z_2$ (sample (q_z2))
      [q_mu1 q_s3] (q-mu (get-$\phi_\mu$ $\phi$) $Y_n$ [$z_1$ $z_2$] q_s2)
      $\mu_1$ (sample (q_mu1))
      [q_mu2 _] (q-mu (get-$\phi_\mu$ $\phi$) $Y_n$ [$z_1$ $z_2$ $\mu_1$] q_s3)
      $\mu_2$ (sample (q_mu2))]
    [$z_1$ $z_2$ $\mu_1$ $\mu_2$]))

;; generative model, p, params 
;; i.e. (def $\theta$ [0.5 0 1 2 1])
(defn get-$\theta_z$  [$\theta$] (get $\theta$ 0))
(defn get-$\theta_{\mu_1}$ [$\theta$] (get $\theta$ 1))
(defn get-$\theta_{\mu_2}$ [$\theta$] (get $\theta$ 2))
(defn get-$\theta_{\sigma_\mu^2}$ [$\theta$] (log (+ 1 (exp (get $\theta$ 3)))))
(defn get-$\theta_{\sigma_y^2}$ [$\theta$] (log (+ 1 (exp (get $\theta$ 4)))))
        
;; generative model p        
(defn generative-model [$\theta$ $Y_n$]
  (let [$z_1$ (sample (bernoulli (get-$\theta_z$ $\theta$)))       
        $z_2$ (sample (bernoulli (get-$\theta_z$ $\theta$)))
        $\mu_1$ (sample (normal (get-$\theta_{\mu_1}$ $\theta$) (get-$\theta_{\sigma_\mu^2}$ $\theta$)))
        $\mu_2$ (sample (normal (get-$\theta_{\mu_2}$ $\theta$) (get-$\theta_{\sigma_\mu^2}$ $\theta$)))]
     (observe (normal (if $z_1$ $\mu_1$ $\mu_2$) (get-$\theta_{\sigma_y^2}$ $\theta$))
              (get $Y_n$ 0))
     (observe (normal (if $z_1$ $\mu_1$ $\mu_2$) (get-$\theta_{\sigma_y^2}$ $\theta$))
              (get $Y_n$ 1))
     [$z_1$ $z_2$ $\mu_1$ $\mu_2$]))
\end{foppl}
%(def $Y$ [[0.5 2]])
%(defn q-z [$\phi$ $Y$ $X$ $S$] $\ldots$)
%(defn q-mu [$\phi$ $Y$ $X$ $S$] $\ldots$)
%;; i.e. (def $\theta$ [0.5 0 1 1])
%(defn get-$\theta_z$  [$\theta$] (get $\theta$ 0))
%(defn get-$\theta_{\mu_1}$ [$\theta$] (get $\theta$ 1))
%(defn get-$\theta_{\mu_2}$ [$\theta$] (get $\theta$ 2))
%(defn get-$\theta_y$  [$\theta$] (get $\theta$ 0))
%;; i.e. (defq $\phi$ [$\ldots$, $\ldots$]) 
%(defn get-$\phi_z$ [$\phi$] (get $\phi$ 0))
%(defn get-$\phi_\mu$ [$\phi$] (get $\phi$ 1))
%(defp $\theta_z$ 0.5)
%(defp $\theta_\mu$ [0 1])
%(defp $\theta_y$ 1)
%(defq $\lambda_z$ $\ldots$)
%(defq $\lambda_\mu$ $\ldots$)


Throughout this chapter we will make use of a simple, pedagogical example in the form of a ``structured'' VAE.  The decoder portion of Program~\ref{foppl:pyro-like-model} consists of a two component normal mixture model of two observations with learnable rather than inferred parameters $\theta$.  It is written in unrolled form, without looping constructs, in order to keep things as clear as possible.  The generative model program should be quite clear in the context of the rest of the book.

The inference network in this example appears complex but is actually quite simple.  It is a recurrent-type neural network that samples the {\em same sequence} of random variables as the generative model, albeit from potentially different distribution types.   The inference network is parameterized by $\phi$, is conditioned on the observation $Y_n$, and passes a state (the $q_s$'s) from one sub-neural-network to the next. Each sub-neural-network has access to all of the previously sampled values.







%    \Comment{}
%    \State \textbf{global} $V,X,Y,\m{P},\m{Y}$
%    \Comment{A directed graphical model}
%    \State \textbf{global} $\m{Q}$
%    \Comment{A map of proposal expressions}
%    \Function{accept}{$x, \m{X}', \m{X}$}
%      \State $d \gets \textsc{eval}(\m{Q}(x)[Y:=\m{Y}, X:=\m{X}])$
%      \State $d' \gets \textsc{eval}(\m{Q}(x)[Y:=\m{Y}, X:=\m{X}'])$
%      \State $\log \alpha \gets \textsc{log-prob}(d', \m{X}(x)) - \textsc{log-prob}(d, \m{X}'(x))$
%      \State $V_{x} \gets \{ v \colon x \in \textsc{free-vars}(\m{P}(v)) \}$
%      \For{$v$ \textbf{in} $V_x$}
%        \State $\log \alpha \gets \log \alpha + \textsc{eval}(\m{P}(v)[Y:=\m{Y}, X:=\m{X}'])$
%        \State $\log \alpha \gets \log \alpha - \textsc{eval}(\m{P}(v)[Y:=\m{Y}, X:=\m{X}])$
%      \EndFor
%      \State \Return $\alpha$
%    \EndFunction
%    \Function{gibbs-step}{$\m{X}$}
%    \For {$x$ \textbf{in} $X$}
%        \State $d \gets \Call{eval}{\m{Q}(x)[Y:=\m{Y}, X:=\m{X}]}$
%        \State $\m{X}' \gets \m{X}$
%        \State $\m{X}'(x) \gets \Call{sample}{d}$
%        \State $\alpha \gets \Call{accept}{x, \m{X'}, \m{X}}$
%        \State $u \sim \text{Uniform}(0,1)$
%        \If{$u < \alpha$}
%           \State $\m{X} \gets \m{X}'$
%        \EndIf
%      \EndFor
%      \State \Return $\m{X}$
%    \EndFunction
%    \Function{gibbs}{$\m{X}^{(0)}, S$}
%    \For {$s$ \textbf{in} $1, \ldots, S$}
%      \State $\m{X}^{(s)} \gets \Call{gibbs-step}{\m{X}^{(s-1)}}$
%    \EndFor
%    \EndFunction
%    \State \Return $\m{X}^{(1)}, \ldots \m{X}^{(S)}$
%    \end{algorithmic}
%    \end{algorithm}





%[z_1 z_2 mu_1 mu_2]

\section*{Organization}

Having established what we want to do (to learn model parameters from big data and be able perform rapid amortized inference), it remains to explain how to do this both in terms of the mathematical operations required and language design consideration.  
The technical part of this chapter, starting now, discusses mathematical techniques that make use of gradient computations to both estimate model parameters and to learn the parameters of amortized inference artifacts. We have already seen two examples of algorithms that use gradients for inference; Hamiltonian Monte Carlo (HMC) in Section~\ref{sec:hmc} and black-box variational inference in Section~\ref{sec:eval-bbvi}. 
 HMC used gradients to construct high quality proposals for MCMC inference, whereas black-box variational inference used gradients to estimate parameters of an approximation to the probabilistic program posterior (a one-shot, non-amortized inference task). 

This chapter takes a more general view of gradient-based methods. It begins by showing how to do maximum likelihood model parameter estimation using stochastic gradient descent.  As we will establish, maximum likelihood parameter estimation requires samples from the program posterior.  This connects to the preceding chapters in the book as any of the probabilistic program inference methods described so far can be used to do this. 

It then discusses model parameter learning in the context of variational inference.  We show how model parameter learning is also evidence lower bound maximization in the variational inference framework and explain how variational approximate posteriors can be used for efficient importance-sampling-based model learning. 

The variational framework also presents opportunities to simultaneously learn model parameters and amortized inference neural network artifacts.  We discuss how this works, showing that amortized inference networks predict approximate variational posterior parameters directly from observations.   We relate amortized variational inference to both wake-sleep and variational autoencoders.

%Amortized vartional methods, which were originally developed in the context of wake-sleep methods and variational autoencoders, are now increasingly used to both train the generative model and accelerate inference in probabilistic programs that are parameterized using neural networks. 
%In Sections~\ref{sec:amortized-inference} and~\ref{sec:advanced-amortized-inference} 
Finally, we discuss the design challenges that arise when constructing inference networks for probabilistic programs, and more generally when implementing deep probabilistic programming systems on top of languages endowed with first class automatic differentiation and optimization primitives.

% TODO: something about PPLs here

%we d look into how this can be used for both faster variational inference than the ``black box'' algorithm of Section~\ref{sec:eval-bbvi}, as well as how we can define more flexible approximating families for more accurate posterior representations.

%After revisiting variational inference, we then consider extensions which incorporate deep learning, for amortizing runtime costs of inference (Section~\ref{sec:advanced-inference-compilation}), and fitting model parameters jointly with performing inference (Section~\ref{sec:amortized-inference}).
%We end the chapter by considering the challenges encountered when implementing Hamiltonian Monte Carlo and variational inference within the HOPPL.


==> sections/deep-probprog-examples.tex <==
%\section{Examples}

\subsection*{Bayesian Neural Networks}
To build some intuition about such ML/AI application characteristics, first refer back to the very simple Bayesian neural network example program in Chapter~\ref{ch:foppl}, Program~\ref{foppl:bnn_edward}, which framed parameter ``learning'' in a neural network as inference in, effectively, a generative model of neural network parameters.  This program generated the weights of a neural network from a standard prior (corresponding to ``weight decay'' or L2 regularization) and observed the output value of a number of input/output observation pairs (corresponding to an L2 regression loss) given the input passed through the neural network.   The input/output relationship of the data inlined in Program~\ref{foppl:bnn_edward} is so simple that it can be deduced directly by simply looking at the data: output equals input squared.  The triviality of this example made writing the program compact and illuminating with respect to the design of the FOPPL but  may have obfuscated the important points that we address in this chapter.  Simply considering a larger scale, generic version of this program/problem will help characterize two of these points.  Consider the pseudo-code in Program~\ref{foppl:generic_bnn}.  This is a generic program that takes a large amount, \mang{N}, of data $Y_1, \ldots, Y_N$ consisting of input/label pairs and generates a posterior distribution over the weights $\theta$ of a neural network. 

\begin{foppl}[mathescape,caption={A Generic Bayesian Neural Network for Classification},label=foppl:generic_bnn,float=tbp,floatplacement=thbp]

(defn sample-weights [] $\ldots$)
(defn neural-network [weights input] $\ldots$)

(let [data [$\ldots$] ;; [[input1 label1] [input2 label2] $\ldots$] 
      N $\ldots$     ;; number of training pairs
      $\theta$ (sample-weights)]
  (foreach N 
    [pair data]
    (let [input (get pair 0)
          label (get pair 1)] 
      (observe 
        (discrete (neural-network $\theta$ input)) 
        label))))  
\end{foppl}

%\begin{foppl}[mathescape,caption={A Generic Bayesian Neural Network for Classification},label=foppl:generic_bnn,float=tbp,floatplacement=thbp]
%
%(defn sample-weights [] $\ldots$)
%
%(defn neural-network [weights input] $\ldots$)
%
%(let [input [$\ldots$]
%      label [$\ldots$]
%      N $\ldots$
%      weights (sample-weights)]
%  (foreach N 
%    [x input 
%     y label] 
%    (observe (discrete (neural-network weights x)) y))
%  weights)  
%\end{foppl}

Program~\ref{foppl:generic_bnn} illustrates two of the characteristics of ML/AI applications.  First, it illustrates conditioning on a large amount of data.  This has ramifications we will consider with respect to whether or not we should treat $\theta$ as a parameter for which we should compute a point estimate or whether we should continue, as we have throughout the entire book until now, to treat it as a latent variable for which we should compute an approximate posterior. And second, the relationship from input to label, particularly if the inputs live in, for instance, the space of images, and the labels live in, for instance, the space of object class identities, is impossible to program manually (whereas it was not just conceivable but even trivial in Program~\ref{foppl:bnn_edward}).   In other words the \mang{neural-network} function which takes  \mang{weights} and \mang{input} and produces, here, softmax weights for the parameters of categorial (or cross-entropy) loss can be thought of as an otherwise impossible to code program fragment; a part of the model which we would like to learn.  %Assume that some architecture of the neural network is given (e.g.~convolutional with three layers, some number of filters, some kind of pooling, etc.), but the parameters of this neural network are not, and what we want/aim to do is to learn the parameters of this program fragment (or distribution over them as is the case thusfar) so that the rest the whole program ``makes sense.''  
This is, in a sense, what model learning is about. 

\subsection*{Model Predictive Control}
%
\begin{foppl}[mathescape,caption={Model-Predictive Control via Inference},label=foppl:generic_rl_state_transition_model,float=tbp,floatplacement=thbp]
;; Markov decision process (MDP)
(defn next-state-dist [$s_t$ $a_t$] $\ldots$ $p(s_{t+1}|s_{t},a_t)$)
(defn reward [$s_t$ $a_t$] $\ldots$)
(defn allowed-action-dist [$s_t$] $\ldots$ $p(a_t|s_{t})$)

(defn step [t s_and_a]
  (let [s (get s_and_a 0)
        a (get s_and_a 1)
        next_s (sample (next-state-dist s a))
        next_a (sample (allowed-action-dist next_s))]
     (observe 
        (bernoulli (exp (- (reward next_s next_a)))) 
        true) ;; $y_t$ =  true
     [next_s next_a]))

(let [$T$ 10 ;; planning horizon
      $a_t$ (sample (allowed-action-dist $s_t$))]
   (observe 
     (bernoulli (exp (- (reward $s_t$ $a_t$))))
     true)
   (loop $T$ [$s_t$ $a_t$] step)
   $a_t$)
\end{foppl}
% ;; assume current state $s_t$ already bound 
% (defn equilibrium-state-dist [$s$] $p(s)$)
%      _ (observe (equilibrium-state-dist) $s_t$)
While Program~\ref{foppl:generic_bnn} highlights the first two AI/ML problem characteristics we address in this chapter, it does not require rapid, repeated inference. Program~\ref{foppl:generic_rl_state_transition_model} does.  This program frames action selection in model predictive control setting as an inference problem.  This program frames the Markov decision process control problem of selecting action $a_t$ when in state $s_t$ via inference in the joint distribution
%
\begin{align}
p(a_t,s_t,&\tau,y_{t:t+T}) = p(s_t)p(a_t|s_t) p(y_t|s_t,a_t) 
\\
& {} \times 
        \prod_{i=1}^{T} 
        p(s_{t+i}|s_{t+i-1},a_{t+i-1})
        p(a_{t+i}|s_{t+i}) 
        p(y_{t+i}|s_{t+i}, a_{t+1}) 
        \nonumber
\end{align} 
%
where $\tau = \{s_{t+1}, a_{t+1}, \ldots, s_{t+T}, a_{t+T}\}$.  Here $Y = \{s_t,y_{t:t+T}\}$ are the observations on which we will condition and $X = \{s_{t+1:t+T},a_{t:t+T}\}$ are the latent variables, the marginal conditional distribution of $a_t$ being of particular interest.  The $y_{t:t+T}$'s are auxiliary Boolean variables that always take the value \mang{true}, and the variables are given distributions with parameters that put the reward in the ``right places'' mathematically speaking in following expressions. The conditional distribution of 
%
\begin{align}
p(&a_t,\tau|s_t, y_{t:t+T} = \vec{\mang{true}}) \\
        &\propto  p(a_t|s_t)e^{r(s_t, a_t)} \prod_{i=1}^{T} 
        p(s_{t+i}|s_{t+i-1},a_{t+i-1})p(a_{t+i}|s_{t+i}) 
        e^{r(s_{t+i}, a_{t+i})} 
        \nonumber
\end{align} 
%
contains the marginal $p(a_t|s_t, y_{t:t+T} = \vec{\mang{true}})$ which is the ``optimal'' distribution over the action to take at time $t$ given an undiscounted ``planning'' horizon of time $T$.  This choice is optimal in the sense that 
\begin{align}
\log p(&a_t|s_t, y_{t:t+T} = \mang{true}) \\
%%&=  {r(s_t, a_t)} + \log \left( \int e^{r(s_{t+i}, a_{t+1})} p(s_{t+i}|s_{t+i-1},a_{t+i-1}) p(a_{t+i}|s_{t+i}) d\tau \right) \\
        &=  \log p(a_t|s_t) + {r(s_t, a_t)}  + \log\left( \mathbb{E}_{p(\tau|a_t,s_t)}\left[\prod_{i=1}^T e^{r(s_{t+i}, a_{t+i})}\right]\right) \label{eq:1bf}\\
        &\geq \log p(a_t|s_t) + {r(s_t, a_t)} + \mathbb{E}_{p(\tau|a_t,s_t)}\left[\sum_{i=1}^T r(s_{t+i}, a_{t+i})\right] \label{eq:1af} \\
        &\approx  \log p(a_t|s_t) + r(s_t, a_t) + Q(s_t,a_t)
\end{align} 
where $p(a_t|s_t)$ is usually the uniform over all choices of $a_t$ and does not affect the optimality, $r(s_t, a_t)$ is the instantaneous reward for taking action $a_t$, and $Q(s_t,a_t)$ is the expected reward ahead, integrating over future states of the world
assuming that you have no a priori preference over subsequent actions and the world transitions according to your model $p(s_{t+1}|s_{t},a_t)$ of it.  We assume positive rewards and use Jensen's inequality to go from \eqref{eq:1bf} to \eqref{eq:1af}.

This application, while a bit involved as an example, directly highlights the most genuine kind of ML/AI application inference runtime requirement.  Of course there are other ways to learn and choose how act in the world besides model-predictive control.   However, any agent that does use inference for model-predictive control for action selection cannot wait around for a long time while an estimate of $p(a_t|s_t,y_{t:t+T})$ is approximated before acting.   And such an agent would need to repeatedly, not just one-time, solve this inference problem.

Careful readers will note that $s_t$ is not bound in Program~\ref{foppl:generic_rl_state_transition_model}.  This is because this is a conditional generative model and it can safely be assumed that this probabilistic program would be executed in a context in which $s_t$ is known and would be provided to the model at inference time.
\subsection*{Variational Autoencoder}

%(defn softplus [x] (log (+ 1 (exp x))))
\begin{foppl}[escapeinside={/*!}{!*/},mathescape,caption={Variational Auto-Encoder},label=foppl:vae,float=tbp,floatplacement=thbp]
;; q, the "encoder"
(defn q-x [$\phi$ $Y_n$] 
  (let [h (nn_q_1 $Y_n$ $\phi$)
        mu (nn_q_2 h $\phi$)
        sigma-sq (vsoftplus (nn_q_3 h $\phi$))]
     (diag-mvn mu sigma-sq)))
     
(defn inference-network [$\phi$ $Y_n$]
  (sample (q-x $\phi$ $Y_n$)))
  
;; p, the "decoder"
(defn generative-model [$\theta$ $Y_n$]
  (let [$X_n$ (sample (diag-mvn $\theta$))
        h (nn_p_1 $X_n$ $\theta$)
        mu (nn_p_2 h $\theta$)
        sigma-sq (softplus (nn_p_3 h $\theta$))]
     (observe (diag-mvn mu sigma-sq) $Y_n$)))          
\end{foppl}

While not an application per se, the variational autoencoder (VAE) model family \citep{rezende2014stochastic,kingma2014auto} arguably is what led to the confluence of probabilistic programming and deep learning which we cover in this chapter.  Variational autoencoders consist of both a generative model which transforms a random vector into a likelihood over some observation space and an amortized inference artifact that performs approximate inference in constant time.  While exactly what this inference network is will not be clear until later in the chapter, you can think of it as replacing the asymptotically convergent inference {\em algorithms} that we have thusfar discussed throughout this book with a constant-time approximate algorithm.  

Program~\ref{foppl:vae} shows program fragments corresponding to both parts of a generic VAE, a generative model or ``decoder'' \mang{p} and an inference network or ``encoder'' \mang{q}.  All variables in Program~\ref{foppl:vae} should be read as being vector valued, \mang{vsoftplus} should be read as the broadcasting of the softplus function $f(x) = \log(1+\exp(x))$ across the dimensions of the argument (i.e., the pointwise application of the softplus to the input vector), all of the \mang{nn_q}'s and \mang{nn_p}'s should be read as neural networks of some structure whose weights are subsets of $\phi$ and $\theta$ respectively, and \mang{diag-mvn} is a multivariate normal distribution with a diagonal covariance matrix whose diagonal elements are given by the vector \mang{sigma-sq}.  For concreteness you could imagine that $Y_n$ is a vectorized, transformed grayscale image and $X_n$ is a, say, 64 dimensional vector.

VAEs bring together all of the characteristics of AI/ML problems in the probabilistic programming context.  The role of the encoder is explicitly to perform rapid amortized inference.  The decoder is a partially specified generative model.  Only the structure of the generative model is provided; the neural network architecture and the choice of prior and likelihood distribution types.  The rest must be learned from data.  And more clearly than any of the previous examples, the very idea of learning generative model parameters from the data requires multiple observations, in many cases ``big data.''  In Program~\ref{foppl:vae} the decoder is in the form of the programs we have seen throughout this text.  Inference in this program would return the posterior distribution over \mang{x} given \mang{y} for each value of $\theta$.  But without some way to do model parameter learning, inference in such a generative model is non-sensical.

Deep probabilistic programming systems can largely accurately be thought of as languages for specifying richly structured variational auto-encoders where both the encoder (also sometimes called a ``guide'') and the generative model are {\em both} considered part of a probabilistic program.

\subsection*{Structured VAE - A Running Pedagogical Example}
\begin{foppl}[mathescape,caption={Non-Interleaved Inference Network and Generative Model},label=foppl:pyro-like-model,float=tbp,floatplacement=thbp]
;; inference network, q, params
;; i.e. (def $\phi$ [$\ldots$, $\ldots$]) 
(defn get-$\phi_z$ [$\phi$] (get $\phi$ 0))
(defn get-$\phi_\mu$ [$\phi$] (get $\phi$ 1))

;; inference network q
(defn q-z [$\phi$ $Y_n$ $X_n$ $S$] $\ldots$)
(defn q-mu [$\phi$ $Y_n$ $X_n$ $S$] $\ldots$)

(defn inference-network [$\phi$ $Y_n$]
  (let 
     [[q_z1 q_s1] (q-z (get-$\phi_z$ $\phi$) $Y_n$ [] nil) 
      $z_1$ (sample (q_z1)) 
      [q_z2 q_s2] (q-z (get-$\phi_z$ $\phi$) $Y_n$ [$z_1$] q_s1)
      $z_2$ (sample (q_z2))
      [q_mu1 q_s3] (q-mu (get-$\phi_\mu$ $\phi$) $Y_n$ [$z_1$ $z_2$] q_s2)
      $\mu_1$ (sample (q_mu1))
      [q_mu2 _] (q-mu (get-$\phi_\mu$ $\phi$) $Y_n$ [$z_1$ $z_2$ $\mu_1$] q_s3)
      $\mu_2$ (sample (q_mu2))]
    [$z_1$ $z_2$ $\mu_1$ $\mu_2$]))

;; generative model, p, params 
;; i.e. (def $\theta$ [0.5 0 1 2 1])
(defn get-$\theta_z$  [$\theta$] (get $\theta$ 0))
(defn get-$\theta_{\mu_1}$ [$\theta$] (get $\theta$ 1))
(defn get-$\theta_{\mu_2}$ [$\theta$] (get $\theta$ 2))
(defn get-$\theta_{\sigma_\mu^2}$ [$\theta$] (log (+ 1 (exp (get $\theta$ 3)))))
(defn get-$\theta_{\sigma_y^2}$ [$\theta$] (log (+ 1 (exp (get $\theta$ 4)))))
        
;; generative model p        
(defn generative-model [$\theta$ $Y_n$]
  (let [$z_1$ (sample (bernoulli (get-$\theta_z$ $\theta$)))       
        $z_2$ (sample (bernoulli (get-$\theta_z$ $\theta$)))
        $\mu_1$ (sample (normal (get-$\theta_{\mu_1}$ $\theta$) (get-$\theta_{\sigma_\mu^2}$ $\theta$)))
        $\mu_2$ (sample (normal (get-$\theta_{\mu_2}$ $\theta$) (get-$\theta_{\sigma_\mu^2}$ $\theta$)))]
     (observe (normal (if $z_1$ $\mu_1$ $\mu_2$) (get-$\theta_{\sigma_y^2}$ $\theta$))
              (get $Y_n$ 0))
     (observe (normal (if $z_1$ $\mu_1$ $\mu_2$) (get-$\theta_{\sigma_y^2}$ $\theta$))
              (get $Y_n$ 1))
     [$z_1$ $z_2$ $\mu_1$ $\mu_2$]))
\end{foppl}
%(def $Y$ [[0.5 2]])
%(defn q-z [$\phi$ $Y$ $X$ $S$] $\ldots$)
%(defn q-mu [$\phi$ $Y$ $X$ $S$] $\ldots$)
%;; i.e. (def $\theta$ [0.5 0 1 1])
%(defn get-$\theta_z$  [$\theta$] (get $\theta$ 0))
%(defn get-$\theta_{\mu_1}$ [$\theta$] (get $\theta$ 1))
%(defn get-$\theta_{\mu_2}$ [$\theta$] (get $\theta$ 2))
%(defn get-$\theta_y$  [$\theta$] (get $\theta$ 0))
%;; i.e. (defq $\phi$ [$\ldots$, $\ldots$]) 
%(defn get-$\phi_z$ [$\phi$] (get $\phi$ 0))
%(defn get-$\phi_\mu$ [$\phi$] (get $\phi$ 1))
%(defp $\theta_z$ 0.5)
%(defp $\theta_\mu$ [0 1])
%(defp $\theta_y$ 1)
%(defq $\lambda_z$ $\ldots$)
%(defq $\lambda_\mu$ $\ldots$)


Throughout this chapter we will make use of a simple, pedagogical example in the form of a ``structured'' VAE.  The decoder portion of Program~\ref{foppl:pyro-like-model} consists of a two component normal mixture model of two observations with learnable rather than inferred parameters $\theta$.  It is written in unrolled form, without looping constructs, in order to keep things as clear as possible.  The generative model program should be quite clear in the context of the rest of the book.

The inference network in this example appears complex but is actually quite simple.  It is a recurrent-type neural network that samples the {\em same sequence} of random variables as the generative model, albeit from potentially different distribution types.   The inference network is parameterized by $\phi$, is conditioned on the observation $Y_n$, and passes a state (the $q_s$'s) from one sub-neural-network to the next. Each sub-neural-network has access to all of the previously sampled values.







%    \Comment{}
%    \State \textbf{global} $V,X,Y,\m{P},\m{Y}$
%    \Comment{A directed graphical model}
%    \State \textbf{global} $\m{Q}$
%    \Comment{A map of proposal expressions}
%    \Function{accept}{$x, \m{X}', \m{X}$}
%      \State $d \gets \textsc{eval}(\m{Q}(x)[Y:=\m{Y}, X:=\m{X}])$
%      \State $d' \gets \textsc{eval}(\m{Q}(x)[Y:=\m{Y}, X:=\m{X}'])$
%      \State $\log \alpha \gets \textsc{log-prob}(d', \m{X}(x)) - \textsc{log-prob}(d, \m{X}'(x))$
%      \State $V_{x} \gets \{ v \colon x \in \textsc{free-vars}(\m{P}(v)) \}$
%      \For{$v$ \textbf{in} $V_x$}
%        \State $\log \alpha \gets \log \alpha + \textsc{eval}(\m{P}(v)[Y:=\m{Y}, X:=\m{X}'])$
%        \State $\log \alpha \gets \log \alpha - \textsc{eval}(\m{P}(v)[Y:=\m{Y}, X:=\m{X}])$
%      \EndFor
%      \State \Return $\alpha$
%    \EndFunction
%    \Function{gibbs-step}{$\m{X}$}
%    \For {$x$ \textbf{in} $X$}
%        \State $d \gets \Call{eval}{\m{Q}(x)[Y:=\m{Y}, X:=\m{X}]}$
%        \State $\m{X}' \gets \m{X}$
%        \State $\m{X}'(x) \gets \Call{sample}{d}$
%        \State $\alpha \gets \Call{accept}{x, \m{X'}, \m{X}}$
%        \State $u \sim \text{Uniform}(0,1)$
%        \If{$u < \alpha$}
%           \State $\m{X} \gets \m{X}'$
%        \EndIf
%      \EndFor
%      \State \Return $\m{X}$
%    \EndFunction
%    \Function{gibbs}{$\m{X}^{(0)}, S$}
%    \For {$s$ \textbf{in} $1, \ldots, S$}
%      \State $\m{X}^{(s)} \gets \Call{gibbs-step}{\m{X}^{(s-1)}}$
%    \EndFor
%    \EndFunction
%    \State \Return $\m{X}^{(1)}, \ldots \m{X}^{(S)}$
%    \end{algorithmic}
%    \end{algorithm}





%[z_1 z_2 mu_1 mu_2]

==> sections/deep-probprog-intro-old.tex <==
% !TEX root =  ../pp-tutorial-ftml-wip.tex

Up to this point in this book we have focused mainly on two things: 1) the probabilistic programming language design space and 2) inference algorithms.  %This chapter shifts focus rather a lot.  
We have more-or-less assumed that there is a fully specified program in which we wish to perform inference and that we will be doing inference once, since we only have one set of observed data.
This is, in fact, true in a variety of circumstances; notably when doing traditional Bayesian statistical analyses of small data or when doing high fidelity simulation-based studies of particular phenomena. We have also assumed that it does not particularly matter how long inference will take, as long as we can produce high-quality inference results given our computational budget. This chapter pushes past these assumptions.


%We have also assumed that it does not really matter how long inference will take.  In particular, we have assumed that we will be doing inference once per program, and that we would like to have algorithms that produce the highest quality inference results possible in such one-time-only inference scenarios.  

In Chapter~\ref{ch:introduction} we motivated the whole of probabilistic programming by suggesting the utility of probabilistic programming languages and techniques for solving modern artificial intelligence (AI) and machine learning (ML) problems.  This chapter builds on what we have developed so far in this book, addressing issues that commonly arise in ML and AI applications.  

In particular, ML and AI applications are typified by several characteristics that are different to those that we have considered so far in our pedagogical examples.  One, ``big data'':  the existence of huge amounts of data; sometimes labeled, sometimes unlabelled, and sometimes partially labeled.  Two, what we will describe as ``non-programmability'':  the idea that, for instance, in many AI and ML applications it is  inconceivable how to write down a fully specified generative program that describes the entire data generation process.   And three, a ``rapid inference'' requirement:  in many if not all interesting AI and ML applications inference will be repeated and must be fast if it is to be valuable at all.  The techniques covered in this chapter address all of these points.

\section{Examples}
\subsection*{Bayesian Neural Networks}
To build some intuition about such ML/AI application characteristics, first refer back to the very simple Bayesian neural network example program in Chapter~\ref{ch:foppl}, Program~\ref{foppl:bnn_edward}, which framed parameter ``learning'' in a neural network as inference in, effectively, a generative model of neural network parameters.  This program generated the weights of a neural network from a standard prior (corresponding to ``weight decay'' or L2 regularization) and observed the output value of a number of input/output observation pairs (corresponding to an L2 regression loss) given the input passed through the neural network.   The input/output relationship of the data inlined in Program~\ref{foppl:bnn_edward} is so simple that it can be deduced directly by simply looking at the data: output equals input squared.  The triviality of this example made writing the program compact and illuminating with respect to the design of the FOPPL but  may have obfuscated the important points that we address in this chapter.  Simply considering a larger scale, generic version of this program/problem will help characterize two of these points.  Consider the pseudo-code in Program~\ref{foppl:generic_bnn}.  This is a generic program that takes a large amount, \mang{N}, of data $Y_1, \ldots, Y_N$ consisting of input/label pairs and generates a posterior distribution over the weights $\theta$ of a neural network. 

\begin{foppl}[mathescape,caption={A Generic Bayesian Neural Network for Classification},label=foppl:generic_bnn,float=tbp,floatplacement=thbp]

(defn sample-weights [] $\ldots$)

(defn neural-network [weights input] $\ldots$)

(let [Y [$\ldots$] ;; [[input1 label1] [input2 label2] $\ldots$] 
      N $\ldots$     ;; number of training pairs
      $\theta$ (sample-weights)]
  (foreach N 
    [$Y_i$ Y]
    (let [input (get $Y_i$ 0)
          label (get $Y_i$ 1)] 
      (observe 
        (discrete (neural-network $\theta$ input)) 
        label)))
  X)  
\end{foppl}

%\begin{foppl}[mathescape,caption={A Generic Bayesian Neural Network for Classification},label=foppl:generic_bnn,float=tbp,floatplacement=thbp]
%
%(defn sample-weights [] $\ldots$)
%
%(defn neural-network [weights input] $\ldots$)
%
%(let [input [$\ldots$]
%      label [$\ldots$]
%      N $\ldots$
%      weights (sample-weights)]
%  (foreach N 
%    [x input 
%     y label] 
%    (observe (discrete (neural-network weights x)) y))
%  weights)  
%\end{foppl}

Program~\ref{foppl:generic_bnn} illustrates two of the characteristics of ML/AI applications.  First, it illustrates conditioning on a large amount of data.  This has ramifications we will consider with respect to whether or not we should treat $\theta$ as a parameter for which we should compute a point estimate or whether we should continue, as we have throughout the entire book until now, to treat it as a latent variable for which we should compute an approximate posterior. And second, the relationship from input to label, particularly if the inputs live in, for instance, the space of images, and the labels live in, for instance, the space of object class identities, is impossible to program manually (whereas it was not just conceivable but even trivial in Program~\ref{foppl:bnn_edward}).   In other words the \mang{neural-network} function which takes  \mang{weights} and \mang{input} and produces, here, softmax weights for the parameters of categorial (or cross-entropy) loss can be thought of as an otherwise impossible to code program fragment; a part of the model which we would like to learn.  %Assume that some architecture of the neural network is given (e.g.~convolutional with three layers, some number of filters, some kind of pooling, etc.), but the parameters of this neural network are not, and what we want/aim to do is to learn the parameters of this program fragment (or distribution over them as is the case thusfar) so that the rest the whole program ``makes sense.''  
This is, in a sense, what model learning is about. 

\subsection*{Model Predictive Control}
%
\begin{foppl}[mathescape,caption={Model-Predictive Control via Inference},label=foppl:generic_rl_state_transition_model,float=tbp,floatplacement=thbp]
;; Markov decision process (MDP)
(defn next-state-dist [$s_t$ $a_t$] $\ldots$ $p(s_{t+1}|s_{t},a_t)$)
(defn reward [$s_t$ $a_t$] $\ldots$)
(defn allowed-action-dist [$s_t$] $\ldots$ $p(a_t|s_{t})$)

(defn step [t s_and_a]
  (let [s (get s_and_a 0)
        a (get s_and_a 1)
        next_s (sample (next-state-dist s a))
        next_a (sample (allowed-action-dist next_s))]
     (observe 
        (bernoulli (exp (- (reward next_s next_a)))) 
        true) ;; $y_t$ =  true
     [next_s next_a]))

(let [$T$ 10 ;; planning horizon
      $a_t$ (sample (allowed-action-dist $s_t$))]
   (observe 
     (bernoulli (exp (- (reward $s_t$ $a_t$))))
     true)
   (loop $T$ [$s_t$ $a_t$] step)
   $a_t$)
\end{foppl}
% ;; assume current state $s_t$ already bound 
% (defn equilibrium-state-dist [$s$] $p(s)$)
%      _ (observe (equilibrium-state-dist) $s_t$)
While Program~\ref{foppl:generic_bnn} highlights the first two AI/ML problem characteristics we address in this chapter, it does not require rapid, repeated inference. Program~\ref{foppl:generic_rl_state_transition_model} does.  This program frames action selection in model predictive control setting as an inference problem.  This program frames the Markov decision process control problem of selecting action $a_t$ when in state $s_t$ via inference in the joint distribution
%
\begin{align}
p(a_t,s_t,&\tau,y_{t:t+T}) = p(s_t)p(a_t|s_t) p(y_t|s_t,a_t) 
\\
& {} \times 
        \prod_{i=1}^{T} 
        p(s_{t+i}|s_{t+i-1},a_{t+i-1})
        p(a_{t+i}|s_{t+i}) 
        p(y_{t+i}|s_{t+i}, a_{t+1}) 
        \nonumber
\end{align} 
%
where $\tau = \{s_{t+1}, a_{t+1}, \ldots, s_{t+T}, a_{t+T}\}$.  Here $Y = \{s_t,y_{t:t+T}\}$ are the observations on which we will condition and $X = \{s_{t+1:t+T},a_{t:t+T}\}$ are the latent variables, the marginal conditional distribution of $a_t$ being of particular interest.  The $y_{t:t+T}$'s are auxiliary Boolean variables that always take the value \mang{true}, and the variables are given distributions with parameters that put the reward in the ``right places'' mathematically speaking in following expressions. The conditional distribution of 
%
\begin{align}
p(&a_t,\tau|s_t, y_{t:t+T} = \vec{\mang{true}}) \\
        &\propto  p(a_t|s_t)e^{r(s_t, a_t)} \prod_{i=1}^{T} 
        p(s_{t+i}|s_{t+i-1},a_{t+i-1})p(a_{t+i}|s_{t+i}) 
        e^{r(s_{t+i}, a_{t+i})} 
        \nonumber
\end{align} 
%
contains the marginal $p(a_t|s_t, y_{t:t+T} = \vec{\mang{true}})$ which is the ``optimal'' distribution over the action to take at time $t$ given an undiscounted ``planning'' horizon of time $T$.  This choice is optimal in the sense that 
\begin{align}
\log p(&a_t|s_t, y_{t:t+T} = \mang{true}) \\
%%&=  {r(s_t, a_t)} + \log \left( \int e^{r(s_{t+i}, a_{t+1})} p(s_{t+i}|s_{t+i-1},a_{t+i-1}) p(a_{t+i}|s_{t+i}) d\tau \right) \\
        &=  \log p(a_t|s_t) + {r(s_t, a_t)}  + \log\left( \mathbb{E}_{p(\tau|a_t,s_t)}\left[\prod_{i=1}^T e^{r(s_{t+i}, a_{t+i})}\right]\right) \label{eq:1bf}\\
        &\geq \log p(a_t|s_t) + {r(s_t, a_t)} + \mathbb{E}_{p(\tau|a_t,s_t)}\left[\sum_{i=1}^T r(s_{t+i}, a_{t+i})\right] \label{eq:1af} \\
        &\approx  \log p(a_t|s_t) + r(s_t, a_t) + Q(s_t,a_t)
\end{align} 
where $p(a_t|s_t)$ is usually the uniform over all choices of $a_t$ and does not affect the optimality, $r(s_t, a_t)$ is the instantaneous reward for taking action $a_t$, and $Q(s_t,a_t)$ is the expected reward ahead, integrating over future states of the world
assuming that you have no a priori preference over subsequent actions and the world transitions according to your model $p(s_{t+1}|s_{t},a_t)$ of it.  We assume positive rewards and use Jensen's inequality to go from \eqref{eq:1bf} to \eqref{eq:1af}.

This application, while a bit involved as an example, directly highlights the most genuine kind of ML/AI application inference runtime requirement.  Of course there are other ways to learn and choose how act in the world besides model-predictive control.   However, any agent that does use inference for model-predictive control for action selection cannot wait around for a long time while an estimate of $p(a_t|s_t,y_{t:t+T})$ is approximated before acting.   And such an agent would need to repeatedly, not just one-time, solve this inference problem.

Careful readers will note that $s_t$ is not bound in Program~\ref{foppl:generic_rl_state_transition_model}.  This is because this is a conditional generative model and it can safely be assumed that this probabilistic program would be executed in a context in which $s_t$ is known and would be provided to the model at inference time.
\subsection*{Variational Autoencoder}

%(defn softplus [x] (log (+ 1 (exp x))))
\begin{foppl}[escapeinside={/*!}{!*/},mathescape,caption={Variational Auto-Encoder},label=foppl:vae,float=tbp,floatplacement=thbp]
;; q, the "encoder"
(defn q-x [$\phi$ $Y_n$] 
  (let [h (nn_q_1 $Y_n$ $\phi$)
        mu (nn_q_2 h $\phi$)
        sigma-sq (vsoftplus (nn_q_3 h $\phi$))]
     (diag-mvn mu sigma-sq)))
     
(defn inference-network [$\phi$ $Y_n$]
  (sample (q-x $\phi$ $Y_n$)))
  
;; p, the "decoder"
(defn generative-model [$\theta$ $Y_n$]
  (let [$X_n$ (sample (diag-mvn $\theta$))
        h (nn_p_1 $X_n$ $\theta$)
        mu (nn_p_2 h $\theta$)
        sigma-sq (softplus (nn_p_3 h $\theta$))]
     (observe (diag-mvn mu sigma-sq) $Y_n$)))          
\end{foppl}

While not an application per se, the variational autoencoder (VAE) model family \citep{rezende2014stochastic,kingma2014auto} arguably is what led to the confluence of probabilistic programming and deep learning which we cover in this chapter.  Variational autoencoders consist of both a generative model which transforms a random vector into a likelihood over some observation space and an amortized inference artifact that performs approximate inference in constant time.  While exactly what this inference network is will not be clear until later in the chapter, you can think of it as replacing the asymptotically convergent inference {\em algorithms} that we have thusfar discussed throughout this book with a constant-time approximate algorithm.  

Program~\ref{foppl:vae} shows program fragments corresponding to both parts of a generic VAE, a generative model or ``decoder'' \mang{p} and an inference network or ``encoder'' \mang{q}.  All variables in Program~\ref{foppl:vae} should be read as being vector valued, \mang{vsoftplus} should be read as the broadcasting of the softplus function $f(x) = \log(1+\exp(x))$ across the dimensions of the argument (i.e., the pointwise application of the softplus to the input vector), all of the \mang{nn_q}'s and \mang{nn_p}'s should be read as neural networks of some structure whose weights are subsets of $\phi$ and $\theta$ respectively, and \mang{diag-mvn} is a multivariate normal distribution with a diagonal covariance matrix whose diagonal elements are given by the vector \mang{sigma-sq}.  For concreteness you could imagine that $Y_n$ is a vectorized, transformed grayscale image and $X_n$ is a, say, 64 dimensional vector.

VAEs bring together all of the characteristics of AI/ML problems in the probabilistic programming context.  The role of the encoder is explicitly to perform rapid amortized inference.  The decoder is a partially specified generative model.  Only the structure of the generative model is provided; the neural network architecture and the choice of prior and likelihood distribution types.  The rest must be learned from data.  And more clearly than any of the previous examples, the very idea of learning generative model parameters from the data requires multiple observations, in many cases ``big data.''  In Program~\ref{foppl:vae} the decoder is in the form of the programs we have seen throughout this text.  Inference in this program would return the posterior distribution over \mang{x} given \mang{y} for each value of $\theta$.  But without some way to do model parameter learning, inference in such a generative model is non-sensical.

Deep probabilistic programming systems can largely accurately be thought of as languages for specifying richly structured variational auto-encoders where both the encoder (also sometimes called a ``guide'') and the generative model are {\em both} considered part of a probabilistic program.

\subsection*{Structured VAE - A Running Pedagogical Example}
\begin{foppl}[mathescape,caption={Non-Interleaved Inference Network and Generative Model},label=foppl:pyro-like-model,float=tbp,floatplacement=thbp]
;; inference network, q, params
;; i.e. (def $\phi$ [$\ldots$, $\ldots$]) 
(defn get-$\phi_z$ [$\phi$] (get $\phi$ 0))
(defn get-$\phi_\mu$ [$\phi$] (get $\phi$ 1))

;; inference network q
(defn q-z [$\phi$ $Y_n$ $X_n$ $S$] $\ldots$)
(defn q-mu [$\phi$ $Y_n$ $X_n$ $S$] $\ldots$)

(defn inference-network [$\phi$ $Y_n$]
  (let 
     [[q_z1 q_s1] (q-z (get-$\phi_z$ $\phi$) $Y_n$ [] nil) 
      $z_1$ (sample (q_z1)) 
      [q_z2 q_s2] (q-z (get-$\phi_z$ $\phi$) $Y_n$ [$z_1$] q_s1)
      $z_2$ (sample (q_z2))
      [q_mu1 q_s3] (q-mu (get-$\phi_\mu$ $\phi$) $Y_n$ [$z_1$ $z_2$] q_s2)
      $\mu_1$ (sample (q_mu1))
      [q_mu2 _] (q-mu (get-$\phi_\mu$ $\phi$) $Y_n$ [$z_1$ $z_2$ $\mu_1$] q_s3)
      $\mu_2$ (sample (q_mu2))]
    [$z_1$ $z_2$ $\mu_1$ $\mu_2$]))

;; generative model, p, params 
;; i.e. (def $\theta$ [0.5 0 1 2 1])
(defn get-$\theta_z$  [$\theta$] (get $\theta$ 0))
(defn get-$\theta_{\mu_1}$ [$\theta$] (get $\theta$ 1))
(defn get-$\theta_{\mu_2}$ [$\theta$] (get $\theta$ 2))
(defn get-$\theta_{\sigma_\mu^2}$ [$\theta$] (log (+ 1 (exp (get $\theta$ 3)))))
(defn get-$\theta_{\sigma_y^2}$ [$\theta$] (log (+ 1 (exp (get $\theta$ 4)))))
        
;; generative model p        
(defn generative-model [$\theta$ $Y_n$]
  (let [$z_1$ (sample (bernoulli (get-$\theta_z$ $\theta$)))       
        $z_2$ (sample (bernoulli (get-$\theta_z$ $\theta$)))
        $\mu_1$ (sample (normal (get-$\theta_{\mu_1}$ $\theta$) (get-$\theta_{\sigma_\mu^2}$ $\theta$)))
        $\mu_2$ (sample (normal (get-$\theta_{\mu_2}$ $\theta$) (get-$\theta_{\sigma_\mu^2}$ $\theta$)))]
     (observe (normal (if $z_1$ $\mu_1$ $\mu_2$) (get-$\theta_{\sigma_y^2}$ $\theta$))
              (get $Y_n$ 0))
     (observe (normal (if $z_1$ $\mu_1$ $\mu_2$) (get-$\theta_{\sigma_y^2}$ $\theta$))
              (get $Y_n$ 1))
     [$z_1$ $z_2$ $\mu_1$ $\mu_2$]))
\end{foppl}
%(def $Y$ [[0.5 2]])
%(defn q-z [$\phi$ $Y$ $X$ $S$] $\ldots$)
%(defn q-mu [$\phi$ $Y$ $X$ $S$] $\ldots$)
%;; i.e. (def $\theta$ [0.5 0 1 1])
%(defn get-$\theta_z$  [$\theta$] (get $\theta$ 0))
%(defn get-$\theta_{\mu_1}$ [$\theta$] (get $\theta$ 1))
%(defn get-$\theta_{\mu_2}$ [$\theta$] (get $\theta$ 2))
%(defn get-$\theta_y$  [$\theta$] (get $\theta$ 0))
%;; i.e. (defq $\phi$ [$\ldots$, $\ldots$]) 
%(defn get-$\phi_z$ [$\phi$] (get $\phi$ 0))
%(defn get-$\phi_\mu$ [$\phi$] (get $\phi$ 1))
%(defp $\theta_z$ 0.5)
%(defp $\theta_\mu$ [0 1])
%(defp $\theta_y$ 1)
%(defq $\lambda_z$ $\ldots$)
%(defq $\lambda_\mu$ $\ldots$)


Throughout this chapter we will make use of a simple, pedagogical example in the form of a ``structured'' VAE.  The decoder portion of Program~\ref{foppl:pyro-like-model} consists of a two component normal mixture model of two observations with learnable rather than inferred parameters $\theta$.  It is written in unrolled form, without looping constructs, in order to keep things as clear as possible.  The generative model program should be quite clear in the context of the rest of the book.

The inference network in this example appears complex but is actually quite simple.  It is a recurrent-type neural network that samples the {\em same sequence} of random variables as the generative model, albeit from potentially different distribution types.   The inference network is parameterized by $\phi$, is conditioned on the observation $Y_n$, and passes a state (the $q_s$'s) from one sub-neural-network to the next. Each sub-neural-network has access to all of the previously sampled values.







%    \Comment{}
%    \State \textbf{global} $V,X,Y,\m{P},\m{Y}$
%    \Comment{A directed graphical model}
%    \State \textbf{global} $\m{Q}$
%    \Comment{A map of proposal expressions}
%    \Function{accept}{$x, \m{X}', \m{X}$}
%      \State $d \gets \textsc{eval}(\m{Q}(x)[Y:=\m{Y}, X:=\m{X}])$
%      \State $d' \gets \textsc{eval}(\m{Q}(x)[Y:=\m{Y}, X:=\m{X}'])$
%      \State $\log \alpha \gets \textsc{log-prob}(d', \m{X}(x)) - \textsc{log-prob}(d, \m{X}'(x))$
%      \State $V_{x} \gets \{ v \colon x \in \textsc{free-vars}(\m{P}(v)) \}$
%      \For{$v$ \textbf{in} $V_x$}
%        \State $\log \alpha \gets \log \alpha + \textsc{eval}(\m{P}(v)[Y:=\m{Y}, X:=\m{X}'])$
%        \State $\log \alpha \gets \log \alpha - \textsc{eval}(\m{P}(v)[Y:=\m{Y}, X:=\m{X}])$
%      \EndFor
%      \State \Return $\alpha$
%    \EndFunction
%    \Function{gibbs-step}{$\m{X}$}
%    \For {$x$ \textbf{in} $X$}
%        \State $d \gets \Call{eval}{\m{Q}(x)[Y:=\m{Y}, X:=\m{X}]}$
%        \State $\m{X}' \gets \m{X}$
%        \State $\m{X}'(x) \gets \Call{sample}{d}$
%        \State $\alpha \gets \Call{accept}{x, \m{X'}, \m{X}}$
%        \State $u \sim \text{Uniform}(0,1)$
%        \If{$u < \alpha$}
%           \State $\m{X} \gets \m{X}'$
%        \EndIf
%      \EndFor
%      \State \Return $\m{X}$
%    \EndFunction
%    \Function{gibbs}{$\m{X}^{(0)}, S$}
%    \For {$s$ \textbf{in} $1, \ldots, S$}
%      \State $\m{X}^{(s)} \gets \Call{gibbs-step}{\m{X}^{(s-1)}}$
%    \EndFor
%    \EndFunction
%    \State \Return $\m{X}^{(1)}, \ldots \m{X}^{(S)}$
%    \end{algorithmic}
%    \end{algorithm}





%[z_1 z_2 mu_1 mu_2]

\section*{Organization}

Having established what we want to do (to learn model parameters from big data and be able perform rapid amortized inference), it remains to explain how to do this both in terms of the mathematical operations required and language design consideration.  
The technical part of this chapter, starting now, discusses mathematical techniques that make use of gradient computations to both estimate model parameters and to learn the parameters of amortized inference artifacts. We have already seen two examples of algorithms that use gradients for inference; Hamiltonian Monte Carlo (HMC) in Section~\ref{sec:hmc} and black-box variational inference in Section~\ref{sec:eval-bbvi}. 
 HMC used gradients to construct high quality proposals for MCMC inference, whereas black-box variational inference used gradients to estimate parameters of an approximation to the probabilistic program posterior (a one-shot, non-amortized inference task). 

This chapter takes a more general view of gradient-based methods. It begins by showing how to do maximum likelihood model parameter estimation using stochastic gradient descent.  As we will establish, maximum likelihood parameter estimation requires samples from the program posterior.  This connects to the preceding chapters in the book as any of the probabilistic program inference methods described so far can be used to do this. 

It then discusses model parameter learning in the context of variational inference.  We show how model parameter learning is also evidence lower bound maximization in the variational inference framework and explain how variational approximate posteriors can be used for efficient importance-sampling-based model learning. 

The variational framework also presents opportunities to simultaneously learn model parameters and amortized inference neural network artifacts.  We discuss how this works, showing that amortized inference networks predict approximate variational posterior parameters directly from observations.   We relate amortized variational inference to both wake-sleep and variational autoencoders.

%Amortized vartional methods, which were originally developed in the context of wake-sleep methods and variational autoencoders, are now increasingly used to both train the generative model and accelerate inference in probabilistic programs that are parameterized using neural networks. 
%In Sections~\ref{sec:amortized-inference} and~\ref{sec:advanced-amortized-inference} 
Finally, we discuss the design challenges that arise when constructing inference networks for probabilistic programs, and more generally when implementing deep probabilistic programming systems on top of languages endowed with first class automatic differentiation and optimization primitives.

% TODO: something about PPLs here

%we d look into how this can be used for both faster variational inference than the ``black box'' algorithm of Section~\ref{sec:eval-bbvi}, as well as how we can define more flexible approximating families for more accurate posterior representations.

%After revisiting variational inference, we then consider extensions which incorporate deep learning, for amortizing runtime costs of inference (Section~\ref{sec:advanced-inference-compilation}), and fitting model parameters jointly with performing inference (Section~\ref{sec:amortized-inference}).
%We end the chapter by considering the challenges encountered when implementing Hamiltonian Monte Carlo and variational inference within the HOPPL.


==> sections/graph-hmc.tex <==
% !TEX root =  ../pp-tutorial-ftml.tex



% Consider a program $q$ in the FOPPL represented by a pair $(\rho,e)$ where 
% $\rho$ is a map from procedures to their definitions
% and $e$ is the main expression of the program $q$. Assume that $q$ is 
% translated to a Bayesian network with continuous densities and
% constant observations. That is,
% \[
%         \rho,\,e \Downarrow G,\,E\qquad G = (V,A,p,o)
% \]
% where all vertices $x$ in $V$ represent continuous random variables on $\R$
% with differentiable densities $p(x)$, and observations $o(y)$ are constants 
% for all $y \in \dom(o)$. Let $O = \dom(o)$, the set of the observed random
% variables, and $S = V \setminus O$, that of the rest. Then, 
% the program $q$ defines a model on the variables $S$ with the following (unnormalised) density $\pi$:
% \begin{equation}
%         \label{eqn:hmc-density}
%         \pi(S) = \prod_{x \in S} p(x) \cdot \prod_{y \in O} \left(p(y)[y := o(y)]\right).
% \end{equation}
% This formula is the product of the density expressions (in our language) 
% for $x$ and $y$ that are stored in $p$. In the case of observed variables $y$, 
% we substitute $o(y)$ for $y$ in the expression $p(y)$. This corresponds to
% evaluating the denisty function of $y$ at the observed value $o(y)$. By our assumption, $\pi(S)$ 
% denotes a function differentiable with respect to every variable in $V$.


Hamiltonian Monte Carlo (HMC) is an MCMC algorithm that makes use of gradients
to construct an efficient MCMC kernel for high dimensional distributions. The
HMC applies to a target density $\pi(X) = \gamma(X) / Z$ of the
general form defined in Equation~\eqref{eq:pp-target}, in which each variable
$x \in X$ is continuous. This unnormalized density is traditionally
re-expressed by defining a \emph{potential energy} function
\begin{align}
    U(X)
    :=
    - \log \gamma(X)
    .
\end{align}
With this definition we can express $\pi(X)$ as
\begin{align}
    \pi(X) = \frac{1}{Z} \exp \left\{ - U(X) \right\}.  
\end{align}
To sample from this distribution, HMC introduces a \emph{momentum} variable $r
\in R$ for each variable in $x \in X$. For these variables we assume a
function $K(R) = -\frac{1}{2} R^\top M^{-1} R$ that is known as the \emph{kinetic
energy} of the system. This energy function defines a Gaussian with zero
mean, and covariance $M$. Together, the potential and kinetic energy define a
target distribution
\begin{align}
\begin{split}
  \pi'(X,R) 
  &= \frac{1}{Z'} \exp\{-U(X) - K(R) \} \\
  &= \frac{1}{Z'} \exp\left\{-U(X) - \frac{1}{2} R^\top M^{-1} R \right\}
\end{split}.
\end{align}
In this extended target density, $R$ is known as an \emph{auxiliary} variable. We observe that $X$ and $R$ are uncorrelated. If we marginalize with respect to $R$, we therefore recover the target density,
\begin{align}
  \pi'(X) &= \int \pi'(X, R) \: dR = \pi(X).
\end{align}
This means that if we generate samples $X^{(s)}, R^{(s)} \sim \pi'(X, R)$ and simply ignore the momentum values $R^{(s)}$, then the values $X^{(s)}$ are samples from the marginal $\pi'(X) = \pi(X)$. In other words, the introduction of the auxiliary variables $R$ does not change the distribution over $X$.  

It is not immediately obvious why introducing auxiliary variables $R$ would
make it easier to generate samples, rather than more difficult. As it turns
out, we can use the auxiliary variables $R$ to propose large moves for
$X$ whilst at the same time ensuring that these moves have a high acceptance
probability. HMC is able to propose these moves by jointly changing $(X,R)$ in
a way that preserves the \emph{Hamiltonian} $H(X, R)$, which describes the total
energy of the system
\begin{align}
  H(X, R) = U(X) + K(R).
\end{align}
By way of physical analogy, an HMC sampler constructs samples by simulating the trajectory of a ``marble'' with position $X$ and a momentum $R$ as it rolls through an energy ``landscape'' defined by $U(X)$. When moving ``uphill'' in the direction of the gradient $\nabla U(X)$, the marble loses momentum. Conversely when moving ``downhill'' (i.e. away from $\nabla U(X)$), the marble gains momentum. By requiring that the total energy $H$ should be constant, we can derive the equations of motion
\begin{align}
  \label{eq:hmc-eq-motion}
  \begin{split}
    \frac{dX}{dt} &= \nabla_R H(X,R) = M^{-1} R,  \\
    \frac{dR}{dt} &= -\nabla_X H(X,R) = - \nabla_X U(X).
  \end{split}
\end{align}
That is, paths of $X$ and $R$ that satisfy the above differential equations
preserve the total energy $H(X,R)$,
\begin{align*}
         \frac{d}{dt}H
        & = (\nabla_R H)^\top \frac{dR}{dt} + (\nabla_X H)^\top \frac{dX}{dt} 
        \\
        & = (\nabla_R H)^\top(-\nabla_X H) + (\nabla_X H)^\top(\nabla_R H) 
        \\
        & = -(\nabla_X H)^\top(\nabla_R H) + (\nabla_X H)^\top(\nabla_R H) 
        \\
        & = 0.
\end{align*}
The essential idea behind HMC is that any reversible proposal for which
$H(X',R') = H(X, R)$ will preserve the probability under the target density.
In other words, if we are able to perfectly integrate the equations of motion
in~\eqref{eq:hmc-eq-motion}, then we can use the simulated trajectory to
propose a sample that can be accepted with probability 1. 

HMC makes use of this idea by iterating between two operations. The first is a
Gibbs update on the momentum $R \sim \pi'(R \mid X)$. Since $X$ and $R$ are
independent, $\pi'(R \mid X) = \pi'(R) = \Normal(0, M)$ is simply a Normal
with 0 mean and covariance $M$. Then, HMC performs numerical intregration to
simulate a trajectory $(X_0=X, R_0=R), \ldots, (X_T,R_T)$ from the equations
in~\eqref{eq:hmc-eq-motion}. The final time point of this trajectory is now used 
as a proposal $(X', R') = (X_T, R_T)$. To account for
any numerical error that may arise from the discretization of the equations of
motion, HMC makes use of a Metropolis-Hastings acceptance ratio
\begin{align*} 
        \alpha 
        & = 
        \min \left\{
          1,  \frac{\pi'(X', R')}{\pi'(X, R)} 
        \right\}
        \\
        & = \min \left\{
          1,  \exp \left \{ - H(X', R') + H(X, R) \right \}  
        \right\}.
\end{align*}

\subsection{Automatic Differentiation}
\label{subsec:ad}

%[\emph{ToDo (JW) Feedback about this section is that it is impenetrable. Edit to clarify. Also do a better job of explainin that Stan is not a FOPPL.}]

% \begin{figure}[!t]
% \begin{center}
%   \includegraphics[width=0.85\textwidth]{figs/ad-overview.pdf}
% \end{center}
% \caption{Reverse-mode AD for the function $f(v_1, v_2) = v_1 v_2 - \sin(v_2)$. Evaluation of the gradient is performed in two steps. The forward pass constructs a computation graph in which nodes correspond to intermediate values $v_3$, $v_4$, and the output $v_5$. For each node, we compute the partial derivatives of the value with respect to its inputs. The reverse pass computes the derivatives of the ouput $f(v_1, v_2) = v_5$ with respect to $v_1$ and $v_2$ by walking the constructed computation graph in the reverse direction to propogate derivatives from each node to its inputs.}
% \end{figure}

The essential operation that we need to implement in order to perform HMC for
either a suitably restricted block proposal in the Metropolis-within-Gibbs FOPPL inference algorithm from Section~\ref{sec:gibbs} of this chapter or another suitably restricted FOPPL-like language \citep{stan_software_2014}.
\begin{align}
  \nabla U(X) = -\nabla \log \gamma(X).
\end{align}
When $\gamma(X)$ is the density associated with a probabilistic program, we must take steps to ensure that this density is \emph{differentiable} at all points $X=\m{X}$ in the support of the distribution, noting that the class of all FOPPL programs includes conditional branching statements which renders HMC incompatible with whole FOPPL program inference.  In Section~\ref{sec:hmc-implementation}, we will further discuss implications this has for the structure of a program, and how this differentiability requirement can be relaxed. For now we will assume that $\gamma(X)$ is indeed differentiable everywhere, and either it refers to a joint $p(Y,X)$ over continuous variables, or we are using HMC as a block Gibbs update to sample a subset of continuous variables $X_\text{b} \subset X$ from the conditional $p(X_\text{b} \mid Y, X \setminus X_\text{b})$.

To compute the gradient for a program with graph $(V,A,\m{P},\m{Y})$ and variables $V = Y \cup X$, we need to compute the partial derivatives with respect to each variable $x \in X$ 
\begin{align}
\begin{split}
\nabla_x U(X)
&=
% -\dd{\log \gamma(X)}{x}
% =
-\dd{\log p(Y,X)}{x}
\\
&=
-\frac{\partial \log p(x \mid \pa(x))}
     {\partial x}
-
\sum_{v: x \in \pa(v)}
-\frac{\partial \log p(v \mid \pa(v))}
     {\partial x}
.
% \\
% &=
% -
% \sum_{x' \in X} 
% \dd{\log p(x' | \pa(x'))}{x}
% -
% \sum_{y \in Y}
% \dd{\log p(y | \pa(y))}{x}
% .
\end{split}
\end{align}
In our graph compilation procedure, we have constructed expressions 
$p(x | \pa(x)) \equiv \m{P}(x)$ and $p(y | \pa(y)) \equiv \m{P}(y)[y:=\m{Y}(y)]$ for each random variable. In order to calculate $\nabla U(X)$ we will first
construct a single expression $E_U$ that represents the potential $U(X) \equiv E_U$ as an explicit sum over the variables $X = \{x_1, \ldots, x_N\}$ and $Y = \{y_1, \ldots, y_M\}$
\begin{align*}
  E_X := & \mang{(+ (log\ $\m{P}(x_1)$)\ $\ldots$\ (log\ $\m{P}(x_N)$))}\\
  E_Y := & \mang{(+ (log\ $\m{P}(y_1)[y_1 := \m{Y}(y_1)]$)\ $\ldots$\ (log\ $\m{P}(y_M)[y_M := \m{Y}(y_M)]$))} \\
  %       & \mang{\ \ \ \ \ \ \ \ \ \ \ (log\ $\m{P}(y_1)[y_1 := \m{Y}(y_1)]$)\ $\ldots$\ (log\ $\m{P}(y_M)[y_M := \m{Y}(y_M)]$)))}
  E_U := & \mang{(* -1.0 (+\ $E_X$\ $E_Y$))}
\end{align*}
% Here $\{x_1, \ldots, x_N\} = X$ and $\{y_1, \ldots, y_M\} = Y$ are arbitrary
% orderings on the random variables in the graph. 
%This means that we can represent the values of unobserved variables $\m{X} := (c_1, \ldots, c_N)$ as a real-valued vector in $\mathbb{R}^N$. 
We can then define pointwise evaluation of the potential function by means of the partial evaluation operation $\textsc{eval}$ after substitution of a map $\m{X}$ of values
\begin{align}
  U(X=\m{X}) := \textsc{eval}(E_U[X := \m{X}]).
\end{align}

To compute the partial derivatives of the potential function, we will use reverse-mode automatic differentiation (AD) \citep{griewank2008evaluating,baydin2015automatic}, which is the technique that forms the basis for modern deep learning systems such as TensorFlow \citep{abadi2015tensorflow}, PyTorch \citep{paszke2017automatic}, MxNET \citep{chen2016mxnet}, and CNTK \citep{seide2016cntk}. 

Reverse-mode AD is a computation in two stages, which is illustrated in Figure~\ref{fig:ad-overview}. During the \emph{forward} pass we construct a \emph{computation graph} in which each node corresponds to a primitive procedure call. For each node we compute the output value of the procedure call, as well as the partial derivative of the output with respect to each of the inputs. During the \emph{backward} pass, we walk the computation graph in the reverse direction starting at the output value. At each node, we apply the chain rule of differentiation to propagate derivatives to parent nodes, which in the deep learning community is often referred to as \emph{backpropagation}. 

There are variety of ways to construct the computation graph. In Section~\ref{sec:factor-graph}, we will show how to compile a Bayesian network to a factor graph. This graph will also contain a node for each primitive procedure application, and an edge for each of its inputs. In this section, we will compute this graph dynamically as a side-effect of the evaluation of an expression $E$ in the target language.

\begin{figure}[!t]
\begin{center}
  \includegraphics[width=0.9\textwidth]{figs/ad-overview.pdf}
\end{center}
\caption{
\label{fig:ad-overview}
Reverse-mode AD for the function $f(v_1, v_2) = v_1 v_2 - \sin(v_2)$. Evaluation of the gradient is performed in two steps. The forward pass constructs a computation graph in which nodes correspond to intermediate values $v_3$, $v_4$, and the output $v_5$. For each node, we compute the partial derivatives of the value with respect to its inputs. The reverse pass computes the derivatives of the ouput $f(v_1, v_2) = v_5$ with respect to $v_1$ and $v_2$ by walking the constructed computation graph in the reverse direction to propogate derivatives from each node to its inputs.}
\end{figure}

Suppose that $E$ contains the free variables $V = \{v_1, \ldots, v_{D}\}$. We can think of this expression as a function $E \equiv F(v_1, \ldots, v_{D})$. Suppose that we wish to compute the gradient of $F$ at values 
\begin{align}
  \m{V} = [v_1 \mapsto c_1, \ldots, v_{D} \mapsto c_{D}].
\end{align}
Our goal is now to to define a gradient operator
\begin{align}
  \textsc{grad}
  \left( 
    \textsc{eval}
    \left(
      F[V := \m{V}]
    \right)
  \right),
\end{align}
which computes the map of partial derivatives 
\begin{align}
  \m{G} := 
  \left[
    v_1 \mapsto  \left. \frac{\partial F(V)}{\partial v_1}\right|_{V=\m{V}},
    \ldots,
    v_{D} \mapsto  \left. \frac{\partial F(V)}{\partial v_{D}}\right|_{V=\m{V}}
  \right].
\end{align} 
Given that $F$ is an expression in the target language, we can solve the problem of differentiating $F$ by defining the derivative of each expression type $E$ recursively in terms of the derivatives of its sub-expressions. To do so, we only need to consider four cases:
\begin{itemize}
  \item[1.] Constants $E = c$ have zero derivatives 
  \begin{equation}
  \label{eq:ad-constant}
  \frac{\partial E}{\partial v_i} = 0.
  \end{equation}
  \item[2.] Variables $E = v$ have derivatives
  \begin{equation}
  \label{eq:ad-variable}
  \frac{\partial E}{\partial v_i}
  = 
  \left\{
  \begin{array}{ll}
  1 & v = v_i, \\
  0 & v \not= v_i.
  \end{array}
  \right.
  \end{equation}
  \item[3.] For if expressions $E = \mang{(if\ $E_1$\ $E_2$\ $E_3$)}$ we can define the derivative recursively in terms of the value $c'_1$ of $E_1$,
  \begin{equation}
  \label{eq:ad-if}
  \frac{\partial E}{\partial v_i}
  = 
  \left\{
  \begin{array}{ll}
  \ifrac{\partial E_2}{\partial v_i} 
  & 
  c'_1 = \mang{true}
  \\
  \ifrac{\partial E_3}{\partial v_i} 
  &
  c'_1 = \mang{false}
  \end{array}
  \right.
  \end{equation}
  \item[4.] For primitive procedure applications $E = $\ang{($f$ $E_1$ $\ldots$ $E_n$)} we apply the chain rule 
  \begin{equation}
  \label{eq:ad-primitive}
  \frac{\partial E}{\partial v_i}
  = 
  \sum_{j=1}^n
  %\left.
  \frac{\partial f(v'_1, \ldots, v'_n)}
       {v'_j}
  %\right|_{v'_1=c'_1, \ldots, v'_n=c'_n}
  %\left.
  \frac{\partial E_j}
       {\partial v_i}.
  %\right|_{v_1=c_1, \ldots, v_{D}=c_{D}}
  \end{equation}
  %where $c'_i$ is the value of the sub-expression $E_i$.
\end{itemize}

\begin{algorithm}[!t]
\caption{
  \label{alg:hmc-lift-ad}
  Primitive function lifting for reverse-mode AD.
}
\begin{algorithmic}[1]
\Function{unbox}{$\ad{v}$}
  \If{$\ad{v} = (c,\_)$}
    \State \Return $c$
    \Comment{Unpack value from $\ad{c}$}
  \Else
    \State \Return $\ad{v}$
    \Comment{Return value as is}
  \EndIf
\EndFunction
\Function{lift-ad}{$f$, $\nabla f$, $n$}
   \Function{$\tilde{f}$}{$\ad{c}_1, \ldots, \ad{c}_n$}
      \State $c_1, \ldots, c_n \gets \Call{unbox}{\ad{c}_1}, \ldots, \Call{unbox}{\ad{c}_n}$ 
      %\State $v \gets \Call{gensym}{\,}$
      \State $c \gets f(c_1, \ldots, c_n)$
      \State $\dot{c}_1, \ldots, \dot{c}_n \gets \nabla f(c_1, \ldots, c_n)$
      \State \Return $(c,((\ad{c}_1, \ldots, \ad{c}_n),(\dot{c}_1, \ldots, \dot{c}_n)))$
   \EndFunction
   \State \Return $\tilde{f}$
\EndFunction
\end{algorithmic}
\end{algorithm}

The first three cases are trivial. This means that we can compute the gradient of any target language expression $E$ with respect to the values of its free variables as long as we are able to calculate the partial derivatives of values returned by primitive procedure applications with respect to the values of the inputs. 

Let us discuss this last case in more detail. Suppose that $f$ is a primitive that accepts $n$ real-valued inputs, and returns a real-valued output $c = f(c_1, \ldots, c_n)$. In order to perform reverse-mode AD, we will replace this primitive with a ``lifted'' variant $\tilde{f}$ such that $\ad{c} = \tilde{f}(\ad{c}_1, \ldots, \ad{c}_n)$ will return a boxed value
\begin{align}
  \ad{c} = (c, ((\ad{c}_1, \ldots, \ad{c}_n), (\dot{c}_1, \ldots, \dot{c}_n))),
\end{align}
which contains the return value $c$ of $f$, the input values $\ad{c}_i$, and the values of  the partial derivatives $\dot{c}_i = \partial f(v_1, \ldots, v_n) / \partial v_i |_{v_1,\ldots,v_n=c_1,\ldots,c_n}$ of the output with respect to the inputs. Algorithm~\ref{alg:hmc-lift-ad} shows pseudo-code for an operation that constructs an AD-compatible primitive $\tilde{f}$ from a primitive $f$ and a second primitive $\nabla f$ that computes the partial derivatives of $f$ with respect to its inputs.


The boxed value $\ad{c}$ is a recursive data structure that we can use to walk the computation graph. Each of the input values $\ad{c}_i$ corresponds to the value of a sub-expression that is either a constant, a variable, or the return value of another primitive procedure application. The first two cases correspond to leaf nodes in the computation graph. In the case of a variable $v$ (Equation~\eqref{eq:ad-variable}), we are at an input where the gradient is 1 for the component associated with $v$, and 0 for all other components. We represent this sparse vector as a map $G=[v \mapsto 1]$. When we reach a constant value (Equation~\eqref{eq:ad-constant}), we don't need to do anything, since the gradient of a constant is 0. We represent this zero gradient as an empty map $G=[\,]$. In the third case (Equation~\eqref{eq:ad-primitive}), we can recursively unpack the boxed values $\ad{c}_i$ to compute gradients with respect to input values, multiply the resulting gradient terms by partial derivatives $\dot{c}_i$, and finally sum over $i$. 

\begin{algorithm}[!t]
\caption{
  \label{alg:hmc-grad}
  Reverse-mode automatic differentiation.
}
\begin{algorithmic}[1]
\State \textbf{global} $\m{G} \gets [\,]$ \Comment{Stores the gradients wrt. variables}
\State \textbf{global} $\m{E} \gets [\,]$ \Comment{Stores the gradients wrt. edges in the graph}
\Function{grad}{$\ad{v}$,$[\ad{v}_1,\ldots,\ad{v}_m]$}
  \Comment{The $(\ad{v},\ad{v}_i)$ are all outgoing edges}
  \State Wait until $\dom(\m{E})$ contains all of $(\ad{v},\ad{v}_1),\ldots,(\ad{v},\ad{v}_m)$
  \State $g \gets 0$
  \Comment{$g$ aggregates the gradients wrt. edges $(\ad{v},\ad{v}_i)$}
  \For{$i$ \textbf{in} $1, \ldots, m$}
    \State $g \gets g + \m{E}(\ad{v},\ad{v}_i)$
  \EndFor
  \Match{$\ad{v}$}
    \Comment{Pattern match against value type}
    \Case{$(c,v)$}
      \Comment{Input value}
      \If{$v \in \text{dom}(\m{G})$}
        \State $\m{G}(v) \gets \m{G}(v) + g$
      \Else
        \State $\m{G}(v) \gets g$
      \EndIf
    \EndCase
    \Case{$(c,((\ad{c}_1, \ldots, \ad{c}_n),(\dot{c}_1, \ldots, \dot{c}_n)))$}
      \Comment{Intermediate value}
      \For{$i$ \textbf{in} $1, \ldots, n$}
        \State $\m{E}(\ad{c}_i,\ad{v}) \gets \dot{c}_i \cdot g$
      \EndFor
    \EndCase
    \Case{$\_$}
      \State Skip
      \Comment{Base case, return zero gradient}
    \EndCase
  \EndMatch
\EndFunction
\end{algorithmic}
\end{algorithm}
%
% Jan-Willem's original description of the reverse-mode AD algorithm
%
%\begin{algorithm}[!t]
%\caption{
%  \label{alg:hmc-grad}
%  Reverse-mode automatic differentiation.
%}
%\begin{algorithmic}[1]
%\Function{grad}{$\ad{v}$}
%  \Match{$\ad{v}$}
%    \Comment{Pattern match against value type}
%    \Case{$(c,v)$}
%      \Comment{Input value}
%      \State \Return $[v \mapsto 1]$ 
%    \EndCase
%    \Case{$(c,((\ad{c}_1, \ldots, \ad{c}_n),(\dot{c}_1, \ldots, \dot{c}_n)))$}
%      \Comment{Intermediate value}
%      \State $\m{G} \gets [\,]$
%      \For{$i$ \textbf{in} $1, \ldots, n$}
%        \State $\m{G}_i \gets \Call{grad}{\ad{c}_i}$
%        \For{$v$ \textbf{in} $\text{dom}(\m{G}_i)$}
%        \If{$v \in \text{dom}(\m{G})$}
%          \State $\m{G}(v) \gets \m{G}(v) + \dot{c}_i \cdot \m{G}_i(v)$
%        \Else
%          \State $\m{G}(v) \gets \dot{c}_i \cdot \m{G}_i(v)$
%        \EndIf
%        \EndFor
%      \EndFor
%      \State \Return $\m{G}$
%    \EndCase
%    \Case{$\_$}
%      \State \Return [\,]
%      \Comment{Base case, return zero gradient}
%    \EndCase
%  \EndMatch
%  % \For{$\ad{c}', \dot{c}'$ \textbf{in} $\tau$}
%  %   \State $v',c',\tau' \gets \ad{c}'$
%  %   \If {$v' \not= \mang{nil}$} 
%  %     \State $G(v') \gets \dot{c} \cdot \dot{c}'$
%  %   \Else
%  %     \State $G\,' \gets \Call{grad}{\ad{c}', \dot{c} \cdot \dot{c}'}$
%  %     \For{$v''$ \textbf{in} $\text{dom}(G\,')$}
%  %       \If{$v'' \not\in \text{dom}(G)$}
%  %         \State $G(v'') \gets 0$
%  %       \EndIf
%  %       \State $G(v'') \gets G(v'') + G\,'(v'') $
%  %     \EndFor
%  %   \EndIf
%  % \EndFor
%  %   \If {$G(\text{parents}) = (\,)$}
%  %     \State $g(G) = \delta(G)$
%  %     \Comment{Parent is a leaf node; add to output}
%  %   \Else
%  %     \For{$G\,', \dot{c}\,'$ \textbf{in} $\ad{c}(\text{parents})$}
%  %       \If{$\ad{c}_p \not\in \text{dom}(\delta)$}
%  %         \State $\delta(\ad{c}_p) \gets 0$
%  %         \Comment{Intialize if needed}
%  %       \EndIf
%  %       \State $\delta(\ad{c}_p) \gets \delta(\ad{c}_p) + \delta(\ad{c}) c_p'$
%  %       \Comment{Backpropagate to parent}
%  %     \EndFor
%  %   \EndIf
%  % \EndFor
%\EndFunction
%\end{algorithmic}
%\end{algorithm}
Algorithm~\ref{alg:hmc-grad} shows pseudo-code for an algorithm that performs the reverse-mode gradient computation. The algorithm describes how to compute the gradient of the whole expression with respect to each node in the computation graph, and involves two global data structues denoted $\m{G}$ and $\m{E}$, each storing the gradient of the expression with respect to a variable $v$ or an edge in the computation graph. In the algorithm, we need to know the variable $v$ that is associated with each of the inputs. In order to ensure that we can track these correspondences we will box an input value $c$ associated with variable $v$ into a pair $\ad{c} = (c, v)$. The gradient computation in Algorithm~\ref{alg:hmc-grad} now pattern matches against values $\ad{c}$ to determine whether the value is an input, or an intermediate value that was returned from a primitive procedure call, or any other value (which has a 0 gradient). 

\begin{algorithm}[!t]
  \caption{
    \label{alg:hmc}
    Hamiltonian Monte Carlo}
  \begin{algorithmic}[1]
    % \Function{leapfrog}{$X_0$, $R_0$, $\nabla U$, $L$, $\epsilon$}
    %     \State $R_{1/2} \gets R_0 - \frac{1}{2} \epsilon \nabla U(R_0)$
    %     \For{$\tau$ in $1, \ldots, L-1$}
    %         \State $X_{\tau} \gets X_{\tau-1} + \epsilon R_{\tau-1/2}$
    %         \State $R_{\tau+1/2} \gets R_{\tau-1/2} - \epsilon \nabla U(X_{\tau})$
    %     \EndFor
    %     \State $X_{L} \gets X_{L-1} + \epsilon R_{L-1/2}$
    %     \State $R_{L} \gets R_{L-1/2} - \frac{1}{2} \epsilon \nabla U(X_L)$
    %     \State \Return $X_L, R_L$
    % \EndFunction
    \State \textbf{global} $X,E_U$
    %\State \textbf{global} $\{x_1, \ldots, x_N\} \gets X$
    %\Comment{Induce any ordering}
    \Function{grad}{$\ad{c}, \dot{c}$}
      \State $\ldots$
      \Comment{As in Algorithm~\ref{alg:hmc-grad}}
    \EndFunction
    \Function{$\nabla U$}{$\m{X}$}
      % \State $[v_1 \mapsto c_1, \ldots, v_N \mapsto c_N] \gets \m{X}$
      %\State $\ad{c}_1, \ldots, \ad{c}_N \gets (c_1, x_1), \ldots, (c_N, x_N)$
      %\Comment{Box input variables}
      % \For{$n$ \textbf{in} $1,\ldots,N$}
      %   \State $\ad{c}_n \gets (x_n,c_n,(\,))$
      %   \Comment{Box AD-variables}
      % \EndFor
      \State $\tilde{U} \gets \Call{eval}{E_U[X := \m{X}]}$
      \State \Return $\Call{grad}{\tilde{U}}$
      %\State \Return $(G(x_1), \ldots, G(x_N))$
    \EndFunction
    \Function{leapfrog}{$\m{X}_0$, $\m{R}_0$, $T$, $\epsilon$}
      \State $\m{R}_{1/2} \gets \m{R}_0 - \frac{1}{2} \epsilon \nabla U(\m{X}_0)$
      \For {$t$ \textbf{in} $1, \ldots, T-1$}
        \State $\m{X}_t \gets \m{X}_{t-1} + \epsilon \m{R}_{t-1/2}$
        \State $\m{R}_{t+1/2} \gets \m{R}_{t-1/2} - \epsilon \nabla U(\m{X}_t)$
      \EndFor
      \State $\m{X}_T \gets \m{X}_{T-1} + \epsilon \m{R}_{T-1/2}$
      \State $\m{R}_{T} \gets \m{R}_{T-1/2} - \frac{1}{2} \epsilon \nabla U(\m{X}_T)$
      \State \Return $\m{X}_T, \m{R}_T$
    \EndFunction
    \Function{hmc}{$\m{X}^{(0)}$, $S$, $T$, $\epsilon$, $M$}
      \For {$s$ \textbf{in} $1, \ldots, S$}
        \State $\m{R}^{(s-1)} \sim \Normal(0, M)$
        % \State $\m{R}_0 \gets \m{R}_0 - \frac{\epsilon}{2} M^{-1} \nabla U(\m{X}_0)$
        \State $\m{X}', \m{R}' \gets \Call{leapfrog}{\m{X}^{(s-1)}, \m{R}^{(s-1)}, T, \epsilon}$
        %\For {$l$ \textbf{in} $1, \ldots, L$}
          %\State $\m{X}_l, \m{R}_l \gets \Call{leapfrog}{\m{X}_{l-1}, \m{R}_{l-1}, \epsilon}$
          % \State $\m{X}_l \gets \m{X}_{l-1} + \epsilon \m{R}_{l-1}$
          % \State $\m{R}_l \gets \m{R}_{l-1} - \epsilon M^{-1} \nabla U(X_0)$
        %\EndFor
        % \State $\m{R}_L \gets \m{R}_L + \frac{\epsilon}{2} M^{-1} \nabla U(\m{X}_L)$
        \State $u \sim \text{Uniform}(0,1)$
        \If{$u < \exp \big(- H(\m{X}', \m{R}') + H(\m{X}^{(s-1)}, \m{R}^{(s-1)}\big))$}
            \State $\m{X}^{(s)} \gets \m{X}'$
        \Else
            \State $\m{X}^{(s)} \gets \m{X}$
        \EndIf
      \EndFor
      \Return $\m{X}^{(1)}, \ldots, \m{X}^{(S)}$
    \EndFunction
  \end{algorithmic}
\end{algorithm}

Given this implementation of reverse-mode AD, we can now compute the gradient of the  potential function in two steps
\begin{align}
  \ad{U} &= \textsc{eval}(E_U[V := \m{V}]),
  \\
  \m{G} &= \textsc{grad}(\ad{U}).
\end{align}

\subsection{Implementation Considerations}
\label{sec:hmc-implementation}

Algorithm~\ref{alg:hmc} shows pseudocode for an HMC algorithm that makes use of automatic differentiation to compute the gradient $\nabla U(X)$. There are a number of implementation considerations to this algorithm that we have thus far not discussed. Some of these considerations are common to all HMC implementations. Algorithm~\ref{alg:hmc} performs numerical integration using a leapfrog scheme, which discretizes the trajectory for the position $X$ to time points at an interval $\epsilon$ and computes a correponding trajectory for the momentum $R$ at time points that are shifted by $\epsilon/2$ relative to those at which we compute the position. There is a trade-off between the choice of step size $\epsilon$ and the numerical stability of the integration scheme, which affects the acceptance rate. Moreover, this step size should also appropriately account for the choice of mass matrix $M$, which is generally set to match the covariance in the posterior expectation $M^{-1}_{ij} \simeq \Ev_{\pi(X)}[x_i x_j] - \Ev_{\pi(X)}[x_i]\Ev_{\pi(X)}[x_j]$. Finally, modern implementations of HMC typically employ a No-U-Turn sampling (NUTS) scheme to ensure that the number of time steps $T$ is selected in a way that minimizes the degree of correlation between samples.




An implementation consideration that is particularly relevant to probabilistic programming is that not all FOPPL programs define densities $\gamma(X)=p(Y, X)$ that are differentiable at \emph{all} points in the space. The same is true for systems like Stan \citep{stan_software_2014} and PyMC3 \citep{salvatier2016probabilistic}, which opt to provide users with an expressive modeling language that includes if expressions, loops, and even recursion. While these systems enforce the requirement that a program defines a density over a set of continuous variables that is known at compile time, they do not enforce the requirement that the density is differentiable. For example, the following FOPPL program would be perfectly valid when expressed as a Stan or PyMC3 model:
\begin{center}
\begin{minipage}{0.9\textwidth}
\begin{foppl}[mathescape,label=model:gmm:hmc]
(let 
  [x (sample (normal 0.0 1.0))
   y 0.5]
  (if (> x 0.0)
    (observe (normal 1.0 0.1) y)
    (observe (normal -1.0 0.1) y)))
\end{foppl}
\end{minipage}
\end{center}
This program corresponds to an unnormalized density
\begin{align*}
  \gamma(x) = \text{Norm}(0.5 ; 1, 0)^{I[x > 0]} \text{Norm}(0.5 ; -1, 0)^{I[x \le 0]} \text{Norm}(x ; 0, 1),
\end{align*}
for which the derivative is clearly undefined at $x=0$, since $\gamma(x)$ is discontinuous at this point.
For these non-differentiable models, the standard correctness argument of HMC no longer applies, and its samples are not guaranteed to be drawn from the correct distributions. 

Extending HMC to non-differentiable models is a topic of active research. Discontinuous HMC~\citep{nishimura2020discontinuous} and reflective HMC~\citep{AfsharD15} are representative outcomes of this research effort so far. Both algorithms, however, work only if the set of non-differentiable points of a density has measure zero, which intuitively means that there are not so many such points. \citet{ZhouGKRYW19} proposes a way to restrict a probabilistic programming language and ensure this measure-zero non-differentibility condition. In the context of the FOPPL, this restriction means that all the random variables are continuous\footnote{This part can be relaxed to the requirement that every discrete random variable can be rewritten in terms of a continuous random variable.}, and all primitive functions are analytic (that is, they have Taylor expansions).

%will rely on the Metropolis-Hastings ratio to accept or reject a proposal. When discontinuities are prevalent, this means that HMC proposals may have a low acceptance probability. 




%This means that HMC will not sample from the correct distribution if we were to naively compute the derivatives at $x\not=0$. Even in cases where the density is continuous, the derivative may not be defined at every point. 

% While it is perhaps relatively obvious that if expressions can give rise to problems, there are even cases where the density is continuous, but the derivative is not, which can also give rise to problems. As an example let us consider this program
% \begin{center}
% \begin{minipage}{0.9\textwidth}
% \begin{foppl}[mathescape,label=model:abs:hmc]
% (let 
%   [x (abs (sample (normal 0.0 0.1)))
%    y 0.5]
%   (observe (normal 0.0 (+ x 0.1) y)))
% \end{foppl}
% \end{minipage}
% \end{center}
% Here we are doing something that looks relatively innocuous. Our program defines a density
% \begin{align}
%   \gamma(x) = \text{Norm}(0.5; 0, |x|+0.1) \text{Norm}(x ; 0, 0.1)
% \end{align}


% In other words, it is easy to define a program that may not satisfy the requirements necessary for HMC. So what are these requirements?  Precisely characterizing them is complex although early attempts are being made \citep{gram2018discontinuous}.
% In practice, to be safe, a program should not contain if expressions that cannot be partially evaluated, all primitive functions must be differentiable everywhere, and cannot contain unobserved discrete random variables. 

%We can detect this condition in our graph compilation procedure, since it leads to an expression $\m{P}(y)$ of the form \ang{(if $\phi$ $E$ 1)}, where $E$ is the expression for the likelihood of the observed variable and $\phi$ is an expression that cannot be partially evaluated, which is to say that it has free variables. Moreover all primitive procedures in the program that return doubles should have a well-defined derivative for all possible inputs. This can be a tricky condition for functions such as $\text{abs}(x)$, for which the derivative is defined at all points except $x=0$. 

%What is not necessarily the case is that a differentiable program must \emph{only} make use of primitives that return numbers. In Algorithm~\ref{alg:hmc-lift-ad}, we assume that $f$ is a primitive with a real-valued output and real-valued inputs. In practice, we can also perform reverse-mode AD on programs which incorporate non-differentiable primitives. However such primitives can once again lead to discontinuities. As an example, suppose that we want to take the gradient of an expression of the form \ang{(get [$\ad{c}_2$ $\ad{c}_3$] $c_1$)}. This case is analogous to the gradient of an if expression \textsc{grad}(\ang{(if $c_1$ $\ad{c}_2$ $\ad{c}_3$)}), which evaluates to either $\textsc{grad}(\ad{c}_2)$ or $\textsc{grad}(\ad{c}_3)$, depending on the value of $c_1$. In the same way, the gradient \textsc{grad}(\ang{(get [$\ad{c}_1$ $\ldots$ $\ad{c}_n$] $k$)}) will evaluate to $\textsc{grad}(\ad{c}_k)$. In general, we can interleave non-differentiable and differentiable operations in this manner, as long as we represent all differentiable values using boxed data structures, but when using HMC this can result in non-differentiable density functions. If one wanted to guarantee that a density is differentiable, one could use partial evalution to eliminate all examples of if expressions and data structure assessors in which the selected element or branch is determinable at compile time. If any if expressions or data structure accessors remain after partial evaluation, then one could issue a warning to this effect.   

% There are also some practical efficiency considerations that we have not discussed. In Algorithm~\ref{alg:hmc-grad} we accumulate gradients from inputs to output by looping over maps $G_i$ and their entries in $v$ at every recursion. In practice, it is more efficient to perform accumulation at this point.

% Since $U(X)
% = \log(\gamma(X))$, this requirement implies that we must be able to calculate
% the derivatives of expression $\m{P}(v)$ with respect to every node $v \in V$
% variable $x \in X$, which 
% expression computes both the value of the expression and that of its
% derivative. STAN is a well-known probabilistic programming language that uses
% this approach. Appendix contains further information about automated
% differentiation.





